Benchmark Design and Prior-independent Optimization

This paper compares two leading approaches for robust optimization in the models of online algorithms and mechanism design. Competitive analysis compares the performance of an online algorithm to an offline benchmark in worst-case over inputs, and prior-independent mechanism design compares the expected performance of a mechanism on an unknown distribution (of inputs, i.e., agent values) to the optimal mechanism for the distribution in worst case over distributions. For competitive analysis, a critical concern is the choice of benchmark. This paper gives a method for selecting a good benchmark. We show that optimal algorithm/mechanism for the optimal benchmark are equal to the prior-independent optimal algorithm/mechanism. We solve a central open question in prior-independent mechanism design, namely we identify the prior-independent revenue-optimal mechanism for selling a single item to two agents with i.i.d. and regularly distributed values. Via this solution and the above equivalence of prior-independent mechanism design and competitive analysis (a.k.a. prior-free mechanism design) we show that the standard method for lower bounds of prior-free mechanisms is not generally tight for the benchmark design program.

==> continuous.tex <==
\subsection{Proof by Continuity}

Since the revenue of second price auction $\mech_1$ for triangle
distribution is 1 and the optimal revenue for the triangle
distribution is $2-\qo$ by \Cref{lem:opt rev}, we denote the
approximation ratio for mechanism $\mech_1$ as $\APX_1(\qo) = 2-\qo$,
which is continuous in $\qo$.  Denoting $\APXR(\qo)$ as the
approximation ratio of the optimal mechanism $\mech_{\ratio}$ for
distribution $\tri_{\qo}$ with $\ratio > 1$, i.e., $\APXR(\qo) =
\max_{\ratio}
\frac{\OPT_{\tri_{\qo}}(\tri_{\qo})}{\mech_{\ratio}(\tri_{\qo})}$.  By
\Cref{clm:rev of r}, the approximation ratio $\APXR(\qo)$ is
continuous in $\qo$ as well.  It is easy to verify that $\APX_1(0) >
\APXR(0)$ while $\APX_1(1) < \APXR(1)$.  By continuity, there exists
$\qo^*$ such that $\APXR(\qo^*) = \APX_1(\qo^*)$.  By numerical
calculation, $\qo^* \approx 0.093105$, and
$$\ratio^* = \argmax_{\ratio} \frac{\OPT_{\tri_{\qo}}(\tri_{\qo})}{\mech_{\ratio}(\tri_{\qo})} \approx 2.446946.$$ 


Given mechanism $\mechaAR$, 
we use $\qo_{\ratio}(\alpha)$ to denote
the monopoly quantile as a function of $\alpha$
for the triangle distribution that maximizes the approximation ratio of mechanism $\mechaAR$, i.e., 
$$\qo_{\ratio}(\alpha) = 
\argmax_{\qo} \frac{\OPT_{\tri_{\qo}}}{\mechaAR(\tri_{\qo})}.$$ 
\begin{claim}\label{clm:continuous}
Given any $\ratio \in [\ratioS, \ratioL]$, 
function $\qo_{\ratio}(\alpha)$ is continuous in $\alpha$ for $\alpha \in [\alphaS, \alphaL]$. 
\end{claim}
By numerical calculation, for any $\ratio \in [\ratioS, \ratioL]$, 
$\qo_{\ratio}(\alphaL) < \qo^* < \qo_{\ratio}(\alphaS)$. 
Therefore, by \Cref{clm:continuous}, there exists $\alpha^*$ such that $\qo_{\ratio^*}(\alpha^*) = \qo^*$. 
By numerical calculation, $\alpha^* \approx 0.8056405$. 
Since mechanism $\mechaARO$ and distribution $\tri_{\qo^*}$ are a pair of best responses to each other, 
mechanism $\mechaARO$ is the prior-independent optimal mechanism for triangle distributions, 
and distribution $\tri_{\qo^*}$ is the one minimizes its approximation ratio. 

\begin{proof}[Proof of \Cref{clm:continuous}]
By \Cref{clm:rev of r} and \Cref{thm:myerson}, 
the approximation ratio of mechanism $\mechaAR$ for triangle distribution $\tri_{\qo}$ is 
\begin{align*}
\APX(\alpha, \ratio, \qo) 
&= \frac{\OPT_{\tri_{\qo}}(\tri_{\qo})}{\alpha\cdot \mech_1(\tri_{\qo}) + (1-\alpha)\mech_{\ratio}(\tri_{\qo})} \\
&= \frac{2-\qo}{\alpha 
+ 
\frac{2\ratio(1-\alpha)}{(1-\qo)(\ratio-1)} 
\left(
\frac{1-\qo}{1-\qo+\qo\ratio}
+
\frac{\ln \left(
\frac{\ratio}{1-\qo+\qo\ratio}
\right)}{1-\ratio}
\right)}
\end{align*}
The approximation ratio is a continuous function of $\alpha, \qo$. 
Therefore, to show that fixing $\ratio$,  
function $\qo_{\ratio}(\alpha)$ is continuous in $\alpha$, 
it is sufficient to show that there is a unique $\qo$ that maximizes $\APX(\alpha, \ratio, \qo)$ 
for $\ratio \in [\ratioS, \ratioL]$ and $\alpha \in [\alphaS, \alphaL]$, 
or equivalently, we show that there is a unique $\qo$ that minimizes
$\sfrac{1}{\APX(\alpha, \ratio, \qo)}$. 
By \Cref{clm:cont in r} and \ref{clm:cont in q}, 
we can discretize the quantile space and numerically verify that 
distributions with monopoly quantiles $\qo \not\in [\qoS, \qoL]$ are suboptimal. 
Therefore, we prove the uniqueness of the maximizer by showing that the second order derivative of 
$\sfrac{1}{\APX(\alpha, \ratio, \qo)}$
is strictly positive for $\qo \in [\qoS, \qoL]$. 
\begin{align*}
\frac{\partial^2 \frac{1}{\APX(\alpha, \ratio, \qo)}}{(\partial \qo)^2}
= &
\frac{4(1-\alpha)\ratio
\left(-\frac{\ratio-1}{(1-\qo+\qo\ratio)^2}
+ \frac{1}{(1-\qo)(1-\qo+\qo\ratio)}
- \frac{\log(\frac{\ratio}{1-\qo+\qo\ratio})}{(\ratio-1)(1-\qo)^2}\right)}
{(\ratio-1)(2-\qo)^2}\\
& + \frac{2(1-\alpha)\ratio
\left(-\frac{(\ratio-1)^2}{(1-\qo+\qo\ratio)^3}
- \frac{\ratio-1}{(1-\qo)(1-\qo+\qo\ratio)^2}
+ \frac{2}{(1-\qo)^2(1-\qo+\qo\ratio)}
+ \frac{2\log(\frac{\ratio}{1-\qo+\qo\ratio})}{(\ratio-1)(1-\qo)^3}\right)}
{(\ratio-1)(2-\qo)}\\
& + \frac{4(1-\alpha)\ratio
\left(-\frac{1}{1-\qo+\qo\ratio}
- \frac{\log(\frac{\ratio}{1-\qo+\qo\ratio})}{(\ratio-1)(1-\qo)}\right) 
+ 2\alpha(\ratio - 1)}
{(\ratio-1)(2-\qo)^3}
% \\
% \geq& \frac{4(1-\ratioS)\ratioL
% \left(-\frac{\ratioL-1}{(1-\qoL+\qoS\ratioS)^2}
% + \frac{1}{(1-\qoL)(1-\qoS+\qoS\ratioS)}
% - \frac{\log(\frac{\ratioL}{1-\qoL+\qoS\ratioS})}{(\ratioS-1)(1-\qoL)^2}\right)}
% {(\ratioS-1)(2-\qoS)^2}\\
% & + \frac{2(1-\ratioS)\ratioS
% \left(-\frac{(\ratio-1)^2}{(1-\qo+\qo\ratio)^3}
% - \frac{\ratio-1}{(1-\qo)(1-\qo+\qo\ratio)^2}
% + \frac{2}{(1-\qo)^2(1-\qo+\qo\ratio)}
% + \frac{2\log(\frac{\ratio}{1-\qo+\qo\ratio})}{(\ratio-1)(1-\qo)^3}\right)}
% {(\ratio-1)(2-\qo)}\\
% & + \frac{4(1-\alpha)\ratio
% \left(-\frac{1}{1-\qo+\qo\ratio}
% - \frac{\log(\frac{\ratio}{1-\qo+\qo\ratio})}{(\ratio-1)(1-\qo)}\right) 
% + 2\alpha(\ratio - 1)}
% {(\ratio-1)(2-\qo)^3}
\end{align*}
By substituting the upper and lower bounds of $\alpha, \ratio, \qo$, 
we know that 
\begin{align*}
\frac{\partial^2 \frac{1}{\APX(\alpha, \ratio, \qo)}}{(\partial \qo)^2} > 0.7
\end{align*}
for $\ratio \in [\ratioS, \ratioL], \alpha \in [\alphaS, \alphaL]$ and $\qo \in [\qoS, \qoL]$,
which concludes the uniqueness of the maximizer and the continuity of function 
$\qo_{\ratio}(\alpha)$. 
\end{proof}



==> learning_v2.tex <==
\section{Prior-free versus Prior-independent Expert Learning}
\label{sec:online-learning}

We consider the binary-reward variant of the canonical online expert
learning problem.

A single player plays a repeated game against Nature for $\horizon$
rounds.  In each round $\round$, each expert~$j$ from a discrete set
$\{1,\ldots,\numexpert\}$ will receive a binary reward
$\vali[\round,j]\in\{0,1\}$ as arbitrarily chosen by Nature.
Specifically, the input space is $\feasibleVals =
[\left\{0,1\right\}^\numexpert]^{\horizon}$.  Before rewards are
realized, the player chooses to ``follow'' a (possibly randomized)
expert for the round, and receives a reward (possibly in expectation)
equal to the reward of the followed expert.  When the round concludes,
the player gets to observe the rewards of all experts, including those
not followed by the player.  The player's algorithm is $\mecha$ which
outputs distributions $\mecha_\round(\vals)$ over experts using only the history
$\left(\vali[1],\ldots,\vali[t-1]\right)$ in each round $\round$.  The
class of all such expert learning algorithms is denoted by $\OLA$ and the performance of expert learning algorithm $\mecha\in\OLA$ on input $\vals$ is:
$$
\mecha(\vals) = 
\sum\nolimits_{\round=1}^{\horizon} \expect[j\sim \mecha_\round(\vals)]{\vali[\round,j]}.
$$





As described in \Cref{sec:prior-free} we can define Bayesian,
prior-independent, and prior-free versions of the expert learning
problem.
We summarize as follows:
\begin{itemize}
\item In the Bayesian model, the optimal algorithm is $\OPT_{\dist}
  = \argmax_{\mecha \in \OLA} \mecha(\dist)$.

  
Consider the following family of {\em independent stationary}
distributions $\ISD$ for the Bayesian variant of the expert learning
problem.  For a distribution $\dist \in \ISD$, each expert
$j$'s reward in each round is a Bernoulli random variable with mean
$f_j$.  The class $\ISD$ is composed of all possible means $f_j\in[0,1]$.  At each round $\round$, the rewards are drawn independently
from each other and from other rounds.  Importantly the distribution
of each expert's reward is identical across rounds.
  For independent stationary distributions $\dist \in \ISD$, the
  optimal algorithm picks the expert with the highest ex ante
  probability $j^* = \argmax_j f_j$ and follows expert $j^*$ in each
  round; its expected performance is $$\optf{\dist} = \horizon\,\max_j f_j.$$

\item In the prior-free model, the optimal algorithm is the one that minimizes regret in worst-case over inputs $\vals \in \feasibleVals$ against a given benchmark $\benchmark$ defined as $$\pfratio^{\benchmark} = \min_{\mecha \in \OLA}\max_{\vals \in \feasibleVals} \benchmark(\vals) - \mecha(\vals).$$

  The \emph{best-in-hindsight} benchmark for any reward profile $\vals
  \in \feasibleVals$ is
  $$\BIH(\vals) = \max\nolimits_{j=1}^{\numexpert} \sum\nolimits_{\round=1}^{\horizon}
  \vali[\round, j].$$
  A typical online analysis measures performance
  in terms of worst-case regret with respect to the best-in-hindsight
  benchmark $\BIH$.

\item In the prior-independent model, the optimal algorithm is the one
  that minimizes regret in worst-case over distributions $\dist \in
  \feasibleDist$ against the optimal algorithm for the distribution
  $$\piratio = \min_{\mecha \in \OLA}\max_{\dist \in \feasibleDist}
  \optf{\dist} - \mecha(\dist).$$

  We will be considering this question for independent stationary
  distributions $\ISD$ where $\optf{\dist}$ is as described above.
\end{itemize}



The goal of this section is as follows.  We are comparing the standard
prior-free analysis framework of minimizing hindsight regret with
respect to the best-in-hindsight action to the prior-independent
analysis framework.  For the prior-independent analysis framework the
family of distributions we consider are ones that are independent
across actions and independent and identical across rounds.  With
respect to this family of distributions the best-in-hindsight
benchmark is normalized.  On the other hand, the prior-independent
optimal algorithm is follow-the-leader.  It is well known that
follow-the-leader lacks the robustness of algorithms that approximate
best-in-hindsight.  In particular, there is an input where
follow-the-leader is very far from best-in-hindsight.

We observe first that the best-in-hindsight benchmark is normalized.
(In fact, it is analogous to the normalized benchmark described by
\citet{HR-08} for evaluating prior-free mechanisms.)  Thus, an
algorithm that is a prior-free approximation of the benchmark is also
a prior-independent approximation algorithm (with the same bound on
regret, cf.\ \Cref{prop:npf=>pi}).

\begin{lemma}
  \label{prop:bihisnorm}
  For inputs from independent stationary distributions $\ISD$, the
  best-in-hindsight benchmark $\BIH$ is normalized, i.e., $\BIH(\dist)
  \geq \optf{\dist}$, $\forall \dist \in \ISD$.
  \end{lemma}
\begin{proof}
  Given $\dist \in \ISD$, the Bayesian optimal algorithm
  $\OPT_{\dist}$ selects the same expert in each round.  The
  best-in-hindsight benchmark selects the single expert that is best
  for the realized input $\vals$.  Thus, for all $\vals \in
  \feasibleVals$, $\BIH(\vals) \geq \OPT_{\dist}(\vals)$.  Taking
  expectations we have the lemma.
\end{proof}

We now show that the natural {\em follow-the-leader} algorithm, which
in every round $\round$ -- always chooses a random expert from the set
of experts with highest score from the first $\round-1$ rounds -- is the
prior-independent optimal algorithm.

\begin{definition}
The \emph{follow-the-leader} algorithm uses the uniform distribution $U$ to choose randomly
from experts with highest total historical reward in each round:
$$\FTL_t(\vals) = U[\argmax\nolimits_j \sum\nolimits_{\round' < \round} \vali[\round',j]].$$
\end{definition}


\begin{theorem}\label{thm:pi learning}
The follow-the-leader algorithm is the prior-independent optimal algorithm.
\end{theorem}

\begin{proof}
Suppose we fix the set of distribution $\{p^{j}\}_{j=1}^n$ and the
adversary can choose the permutation~$\permute$ of the experts such
that the distribution for expert $j$ is $f_j = p^{\permute(j)}$.  We
prove \Cref{thm:pi learning} by first proving a stronger result showing that
follow-the-leader is prior-independent for any fixed set of
distributions $\{p^{j}\}_{j=1}^n$.

First note that both the expected optimal reward and the expected
reward of follow-the-leader is invariant of the permutation.
Therefore, any permutation can be the worst case permutation for
follow-the-leader.  Consider the case when the adversary chooses a
uniform distribution over all possible permutations.  The best
algorithm that is aware of this uniform distribution is to form a
posterior of the experts using Bayesian updating given the rewards in
the history, and chooses the expert with highest expectation given the
posterior at each round $\round$.  Note that this algorithm makes
exactly the same (random) choice as follow-the-leader for every
realization of the rewards.  That is, follow-the-leader is optimal for
this adversarial distribution.  By duality, we know that
follow-the-leader is prior-independent optimal when adversary chooses
the permutation.  The optimality of follow-the-leader for general
adversary can be shown by setting of distribution $\{p^{j}\}_{j=1}^n$
as the regret maximization distribution for the follow-the-leader
algorithm.
\end{proof}

As we have proved in \Cref{sec:prior-free}, benchmark
optimization~\eqref{eq:resolution} and prior-independent
optimization~\eqref{eq:pi} are the same.  Thus, the optimal prior-free
benchmark is the performance of follow-the-leader algorithm scaled up by
its prior-independent approximation factor.  Moreover, the optimal
mechanism for the optimal benchmark is the best-in-hindsight algorithm
itself.  If we are hoping for prior-free analysis to be more robust
than prior-independent analysis, by optimizing benchmarks in the
framework provided in \Cref{sec:prior-free}, we have lost all of this
robustness.  Specifically, prior-free approximation of the
best-in-hindsight benchmark admits some robustness that the
follow-the-leader lacks.  This is formalized in the following lemma
which contrasts with the optimal regret of standard algorithms like
randomized weighted-majority \citep{LW-94}.  The optimal worst-case regret against
best-in-hindsight is $\Theta(\sqrt{\horizon \ln \numexpert})$ for
$\numexpert$ experts, $\horizon$ rounds, and binary rewards. \citep{HKW-95}.


\begin{lemma}
  The prior-free regret of follow-the-leader against the
  best-in-hindsight benchmark with $\horizon$ rounds is $\Theta(n)$.
\end{lemma}

\begin{proof}
  Consider the input with an even number of rounds and rounds alternating as:
  \begin{itemize}
  \item odd round payoffs: $(1,0,\ldots,0) \in \{0,1\}^\numexpert$,
  \item even round payoffs: $(0,1,\ldots,1)\in \{0,1\}^\numexpert$.
  \end{itemize}

  The follow-the-leader algorithm chooses a uniform random expert for odd rounds
  and obtains expected payoff $\frac{1}{\numexpert}$ and chooses expert 1 for
  even rounds and obtains expected payoff of $0$.  The total expected
  payoff of follow the leader is $\FTL(\vals) = \frac{\horizon}{\numexpert}$. 
%
  On the other hand, the best-in-hindsight benchmark is $\BIH(\vals) = \frac{n}{2}$.  The additive regret is $\BIH(\vals) - \FTL(\vals) = \frac{n}{2}(1-\frac{1}{k}) \in \Theta(n)$.
\end{proof}

The observations of this section suggest that further study of
benchmark optimization is necessary to better understand the tradeoffs
between prior-free and prior-independent robustness.

%GIVE LOWER BOUND INSTANCE WHERE FOLLOW-THE-LEADER HAS HIGH REGRET WRT BEST-IN-HINDSIGHT.

%I think the worst input is

%(1 0 ... 0) => 1/n
%(0 1 ... 1) => 0
%(1 0 ... 0) => 1/n
%(0 1 ... 1)
%...

%Where FTL gets T/2n and BIH gets T/2 for

%Despite the poor performance of follow-the-leader in worst case, from \Cref{thm:equiv} we have the following positive corollary.

%\begin{corollary}
%\label{cor:ftlsolvesgamma}
%For the expert learning setting with $\numexpert$ experts, finite horizon $\horizon$, and payoffs from $\{0,1\}$, the algorithm with smallest approximation fa%ctor to any normalized benchmark is follow-the-leader.
%\end{corollary}





==> notes/goal.tex <==
\section{Goals}

Missing in paper:
\begin{enumerate}
\item Scale invariance. 
\item Prior-independent optimal auction for $n\geq 3$. 
\end{enumerate}


Other problems:
\begin{enumerate}
\item Algorithmic solution for finding prior-independent optimal auctions. 
\item Solving and motivating program $\pfratio^{\benchmark}$. 
\item Situation when $\pfratio^{\benchmark} = \resolution$.
\item Robustness.
\end{enumerate}



==> notes/notes.tex <==
\section*{Notes}
Prior Independent Optimal Auction

\begin{enumerate}

\item Consider the program 
$$
\max_{\dist \in \tri} \min_{r \geq 1}
\frac{\OPT(\dist)}{\Rev{\mecha_r, \dist}},
$$
the optimal distribution is $\tri_{\quant^*}$ with $\quant^* \approx 0.093$,
and the optimal mechanism is posting second price or
posting second price times $\ratio^* \approx 2.447$. 
This lower bounds the approximation ratio of prior independent mechanism. 

\item For scale invariant look ahead mechanism that posts second price with probability at least $\sfrac{1}{2}$,
the worst case distribution 
truncate the value with non-negative virtual value.

\item For any mechanism that posts second price with probability at least $\sfrac{1}{2}$, and
posts second price times $\ratio$
with the rest probability, 
the worst case distribution is a quadrilateral distribution. 

\item There exists an $\alpha \approx 0.806$ such that 
for posting second price with probability $\alpha$ and
posting second price times $\ratio^*$ with probability $(1-\alpha)$, 
the worst case distribution is triangle distribution with monopoly quantile $\quant^*$. 
This is the optimal scale invariant prior independent mechanism by duality. 

\end{enumerate}

Prior Free Optimal Auction
\begin{enumerate}
\item 
Let $\normBenchmark$ be the set of normalized benchmark for family of distribution $\feasibleDist$, 
\begin{equation*}
\min_{\benchmark\in \normBenchmark} \min_{\mecha \in \feasibleMecha} \max_{\vals} 
\frac{\benchmark(\vals)}{\obj(\mecha, \vals)}
= 
\min_{\mecha \in \feasibleMecha} \max_{\dist \in \feasibleDist} 
\frac{\OPT(\dist)}{\expect[\vals\sim \dist]{\obj(\mecha, \vals)}}.
\end{equation*}

\item
Considering the heuristic approach that optimizes resolution according to the following program 
\begin{align*}
\rho = 
\min_{\benchmark\in \normBenchmark} \max_{\dist \in \feasibleDist} 
\frac{\expect[\vals\sim \dist]{\benchmark(\vals)}}{\OPT(\dist)},
\end{align*}
we have a benchmark that shows a strict separation. 
\end{enumerate}




==> old-files/adversary.tex <==

\section{First Analysis of the Adversary}
\label{s:adversary}

\begin{prop}
Given the {\em prior independent} setting of a revenue auction with 2 agents and an unknown regular distribution $F$, in the mixed-Nash game  interpretation of the question using Yao's $\min-\max$ Theorem, the adversary does not put positive density on any dominated distribution.  Consequently,
\begin{equation}
    \max_{\mathcal{M}}\min_F \mathbf{E}_{v_1,v_2\sim F} \left[\frac{\mathcal{M}(\vecbv)}{\text{OPT}_F(\vecbv)} \right]= \max_{\mathcal{M}}\min_F  \frac{\mathbf{E}_{v_1,v_2\sim F}\left[\mathcal{M}(\vecbv)\right]}{\mathbf{E}_{v_1,v_2\sim F}\left[\text{OPT}_F(\vecbv)\right]}
\end{equation}
\end{prop}


\begin{prop}
Given the {\em prior independent} setting of a revenue auction with 2 agents and an unknown regular distribution $F$.  Define a sub-class of such distributions by its peak revenue point $(q,R)$ in the revenue curve graph (with quantile $q$ on the $x$-axis), and by the shape of the (regular) revenue curve to the right of the peak.  Assume the mechanism $\mathcal{M}$ is unbiased- i.e., it is a lookahead auction which is scale invariant in $v_{\{2\}}$.  The adversary achieves a ratio $\frac{\mathbf{E}_{v_1,v_2\sim \Delta}\left[\mathcal{M}(\vecbv)\right]}{\mathbf{E}_{v_1,v_2\sim \Delta}\left[ \text{OPT}_{\Delta}(\vecbv)\right]}$ in this class using the distribution $\Delta$ represented by truncating all values larger than $R/q$ and putting a point mass with weight $q$ on value $R/q$.
\end{prop}

Alternative form of statement of the previous proposition.


\begin{prop}
Consider any {\em unbiased} auction algorithm \texttt{ALG}.  For the class of distributions characterized by a fixed peak revenue point $(q,R)$ in the ``revenue-curve plane," the prior independent adversary (restricted to the class of regular distributions, versus DSIC auctions) strictly prefers either the triangle revenue curve with peak $(q,R)$ or the point mass distribution at value $R/q$, in comparison to each other element of the class.strictly prefers the triangle revenue curve with peak $(q,R)$ over any other element of the class.
\end{prop}
\begin{proof}
We will show that- holding the rest of the distribution fixed, the adversary strictly prefers to truncate the distribution at $\tau= R/q$, creating the ``left side" of the triangle as a line-segment from $(0,0)$ to the peak.  Second we will show that- again holding the behavior at truncation and now smaller quantiles fixed- the adversary strictly prefers the distribution below the truncation point (in value / price space) to be the constant-negative-virtual-value distribution (CNVV) with virtual value equal to $-R/(1-q)=-\tau q/(1-q)$, creating the ``right side" of the triangle as a line-segment from the peak to $(1,0)$.

For the first part, we give an analysis of the ratio of revenue performances between the optimal algorithms (knowing the regular distribution $\Gamma$ and the truncated (``half-triangle) distribution $\Delta$) and the unbaised algorithm \texttt{ALG}, for both distributions.  Let $P_{q^2}^F\geq 0, ~P_{1-q^2}^{F}\geq 0$ be the revenues that the algorithm gets when it posts its random price above $v_{\{2\}}$ versus distribution $F$ (i.e., the random price it draws is not realized as the point mass on $v_{\{2\}}$), respectively when both value draws are realized to have quantile smaller than $q$ (with probability $q^2$), and otherwise (with probability $1-q^2$).
\begin{align*}
\intertext{For the original arbitrary, fixed regular distribution $\Gamma$ (with peak at $(q,R)$):}
    &\frac{\texttt{OPT}_{\Gamma}}{\texttt{ALG}_{\Gamma}}
    = \frac{\left[\text{Rev}(\texttt{OPT}_{\Gamma})|q_{\{2\}}\leq q\right]+\left[\text{Rev}(\texttt{OPT}_{\Gamma})|q_{\{1\}}\leq q,~q_{\{2\}}\geq q\right]+\left[\text{Rev}(\texttt{OPT}_{\Gamma})|q_{\{1\}}> q\right]}{\left[\text{Rev}(\texttt{ALG}_{\Gamma})|q_{\{2\}}\leq q\right]+\left[\text{Rev}(\texttt{ALG}_{\Gamma})|q_{\{2\}}> q\right]}\\
    &=\frac{\left[q^2\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}\geq \tau\right]\right]+\left[2q(1-q)\cdot \tau\right] +\left[(1-q)^2\cdot0\right]}{\left[q^2\left(\alpha\cdot\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}\geq \tau\right]+P_{q^2}^{\Gamma}\right)\right]+\left[((1-q^2)\left(\alpha\cdot\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}< \tau\right]+P_{1-q^2}^{\Gamma}\right)\right]}\\
\intertext{we re-arrange and conveneniently label quantities:}
&=\frac{\left[A'=q^2\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}\geq \tau\right]\right]+\left[B'=2q(1-q)\cdot \tau\right]}{\left[A''=q^2\left(\alpha\cdot\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}\geq \tau\right]\right)\right]+\left[B''=q^2\cdot P_{q^2}^{\Gamma}+((1-q^2)\left(\alpha\cdot\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}< \tau\right]+P_{1-q^2}^{\Gamma}\right)\right]}\\
\intertext{and for the truncated half-triangle distribution $\Delta$:}
& \frac{\texttt{OPT}_{\Delta}}{\texttt{ALG}_{\Delta}} = \frac{\left[\text{Rev}(\texttt{OPT}_{\Delta})|q_{\{2\}}\leq q\right]+\left[\text{Rev}(\texttt{OPT}_{\Delta})|q_{\{1\}}\leq q,~q_{\{2\}}\geq q\right]+\left[\text{Rev}(\texttt{OPT}_{\Delta})|q_{\{1\}}> q\right]}{\left[\text{Rev}(\texttt{ALG}_{\Delta})|q_{\{2\}}\leq q\right]+\left[\text{Rev}(\texttt{ALG}_{\Delta})|q_{\{2\}}> q\right]}\\
&= \frac{\left[q^2\cdot\tau\right] + \left[2q(1-q)\tau\right]+\left[(1-q)^2\cdot 0\right]}{\left[\alpha q^2\cdot\tau\right]+\left[((1-q^2)\left(\alpha\cdot\mathbf{E}_{\Delta}\left[v_{\{2\}}|v_{\{2\}}< \tau\right]+P_{1-q^2}^{\Delta}\right)\right]}\\
\intertext{again adding some labels:}
&= \frac{\left[C'=q^2\cdot\tau\right] + \left[2q(1-q)\tau\right]}{\left[C''=\alpha q^2\cdot\tau\right]+\left[((1-q^2)\left(\alpha\cdot\mathbf{E}_{\Delta}\left[v_{\{2\}}|v_{\{2\}}< \tau\right]+P_{1-q^2}^{\Delta}\right)\right]}\\
\intertext{and we are interested in the ratios:}
& A=\frac{A'}{A''},~~ B=\frac{B'}{B''},~~C=\frac{C'}{C''}
\end{align*}

Note that after reducing, $A=C=1/\alpha$, though $A$ has numerator $A'$ and denominator $A''$ multiplied by the constant ``heavier weight," i.e., obviously the weight as [(second price) revenue conditioned on $v_{\{2\}}$ at least the Myerson price $\tau$] is at least the weight as [truncation value $\tau$].

Now we consider two cases as $A\geq B$ and $A\leq B$.  For the first case, notice that in fact $A=C=1/\alpha$ is the exact ratio that would be obtained by a point mass distribution at $\tau$, so when $A\geq B$ it follows that the ratio $\texttt{OPT}/\texttt{ALG}$ will be larger using the point mass distribution compared to using $F$.  For the second case, the ratio gets larger replacing $A', A''$ with $C',C''$ respectively- because as mentioned the multiplier is heavier in the $A$ ratio and the total ratio increases when $A\leq B$ and the ``weight" on $A$ decreases:
\begin{align*}
&\frac{\texttt{OPT}_{\Gamma}}{\texttt{ALG}_{\Gamma}}= \frac{\left[q^2\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}\geq \tau\right]\right]+\left[2q(1-q)\cdot \tau\right] }{\left[q^2\left(\alpha\cdot\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}\geq \tau\right]\right)\right]+\left[q^2\cdot P_{q^2}^{\Gamma}+((1-q^2)\left(\alpha\cdot\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}< \tau\right]+P_{1-q^2}^{\Gamma}\right)\right]}\\
& \leq \frac{\left[q^2\cdot\tau\right]+\left[2q(1-q)\cdot \tau\right] }{\left[q^2\left(\alpha\cdot\tau\right)\right]+\left[q^2\cdot P_{q^2}^{\Gamma}+((1-q^2)\left(\alpha\cdot\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}< \tau\right]+P_{1-q^2}^{\Gamma}\right)\right]}\\
&\leq \frac{\left[q^2\cdot\tau\right]+\left[2q(1-q)\cdot \tau\right] }{\left[q^2\left(\alpha\cdot\tau\right)\right]+\left[((1-q^2)\left(\alpha\cdot\mathbf{E}_{\Gamma}\left[v_{\{2\}}|v_{\{2\}}< \tau\right]+P_{1-q^2}^{\Delta}\right)\right]}=\frac{\texttt{OPT}_{\Delta}}{\texttt{ALG}_{\Delta}}
\end{align*}
with the other differences in terms handled trivially in the second inequality because the denominator can only get smaller by $P_{q^2}^{\Gamma}\geq 0$ and $P_{1-q^2}^{\Gamma}\geq P_{1-q^2}^{\Delta}$.
\end{proof}

\begin{prop}
Consider a revenue auction setting with $2$ agents drawn i.i.d. from a regular distribution $F$.  The optimal prior independent auction must be a {\em lookahead} auction.
\end{prop}
\begin{proof}
Since second price auction achieves approximation ratio 2, 
the approximation ratio of the optimal lookahead mechanism is at most 2. 
Hence, 
the optimal lookahead mechanism must post second price with probability at least $\sfrac{1}{2}$. 
Otherwise, 
for the distribution which is a point mass,
the approximation ratio is strictly larger than 2. 
Therefore, by \Cref{...}, we have
\begin{eqnarray*}
&&\max_{\mecha \in \Delta(\la)}
\min_{\dist \in \regular}\Rev{\mecha, \dist}
= \max_{\mecha \in \Delta(\la)}
\min_{\dist \in \tri}\Rev{\mecha, \dist} \\
&=& \min_{\dist \in \Delta(\tri)}
\max_{\mecha \in \la}
\Rev{\mecha, \dist}
= \min_{\dist \in \Delta(\tri)}
\max_{\mecha}
\Rev{\mecha, \dist} \\
&\geq& \min_{\dist \in \Delta(\regular)}
\max_{\mecha}
\Rev{\mecha, \dist}
= \max_{\mecha}
\min_{\dist \in \regular}
\Rev{\mecha, \dist}
\end{eqnarray*}

The second and the last equality holds by min-max theorem. 
The third equality holds because for any mechanism $\mecha$, 
there exists a lookahead mechanism $\mecha'$ 
such that the allocation of the agent with strictly lower value is 0, 
which implies that the expected virtual value of $\mecha'$ is weakly higher, 
and the revenue of $\mecha'$ is weaker higher for all 
triangle distributions. 
The inequality holds since the distribution is chosen from a larger set. 

Since we know that 
$\max_{\mecha}
\min_{\dist \in \regular}
\Rev{\mecha, \dist} 
\geq \max_{\mecha \in \Delta(\la)}
\min_{\dist \in \regular}\Rev{\mecha, \dist}$. 
Combining the two inequalities, 
we have 
\begin{equation*}
\max_{\mecha}
\min_{\dist \in \regular}
\Rev{\mecha, \dist} 
= \max_{\mecha \in \Delta(\la)}
\min_{\dist \in \regular}\Rev{\mecha, \dist}.
\qedhere
\end{equation*}
\end{proof}


% \begin{proof}[sketch]
% The statement follows from the previous proposition, and then the fact that any price offered to the smaller agent with a chance of trading sometimes allocates to a (smaller of the two) agent who has strictly negative virtual value.
% \end{proof}

==> old-files/auction.tex <==

\section{First Analysis of the Auction}
\label{s:auction}

% \begin{prop}
% Consider two different distributions for agents, $F$ and $F'$ such that drawing the revenue curve in quantile space, $F$ has pointwise larger revenue than $F'$ for every input $q\in[0,1]$.  For a constant mechanism $\mathcal{M}$ independent of $n$ agents' randomly drawn values from a fixed distribution (either $F$ or $F'$), the mechanism gets more revenue agents with distribution $F$ than agents with distribution $F'$.
% \end{prop}
% \begin{proof}
% For any fixed mechanism $\mathcal{M}$- i.e., a fixed pricing scheme independent of online information like partial descriptions of agents' values $\valsmi$- for any price posted by $\mathcal{M}$, it sells with weakly smaller probability when the revenue curve is $F$ compared to $F'$, by their descriptions.  This pointwise analysis of ``revenue dominance" is sufficient because $\mathcal{M}$ uses the same distribution over prices regardless of the distributional input, by assumption.
% \end{proof}

% In this section, we will focus on the family of scale invariant mechanism. 
% For each agent $i$, an allocation rule $\alloc_i(v_i, v_{-i})$ is scale invariant if and only if
% for any $\alpha > 0$, $\alloc_i(\alpha v_i, \alpha v_{-i}) = \alloc_i(v_i, v_{-i})$. 
% By the characterization in \citet{...}, 
In this section, we will focus on the family of scale invariant lookahead mechanisms. 
Note that the scale invariant lookahead mechanism can only post price $\ratio \cdot \vsec$
to the highest bidder, where $\ratio \geq 1$ and $\vsec$ the value of the second highest agent. 
Since for scale invariant lookahead mechanism, the mechanism is uniquely determined by the factor $\ratio$, 
we use $\mech_\ratio$ to represent such a mechanism. 
Given that the mechanism is scale invariant, 
both the revenue of the mechanism and the optimal revenue 
increase linearly with respect to the scale. 
Thus, it is sufficient for us to consider the distribution 
such that the single agent optimal revenue is normalized to 1. 
First, we consider the optimal strategy for the adversary. 

\begin{theorem}\label{thm:upper}
Given that the mechanism is scale invariant, 
and the distribution is triangle distribution, 
the worst case distribution is $\tri_{\quant^*}$, 
i.e., $\tri_{\quant^*} = \arg
\min_{\dist \in \tri}
\max_{r \geq 1}\Rev{\mecha_r, \dist}$. 
The corresponding optimal mechanisms are second price auctions, 
or the mechanism which posts $r^* \cdot \vsec$ to the highest bidder. 
By numerical experimentation, 
$\quant^* \approx 0.093, r^* \approx 2.447$, 
and the approximation ratio is $1.907$.
% \footnote{The numbers in the distribution, the mechanism, and the approximation ratio are all numerical solutions. }
\end{theorem}
\begin{proof}
For any triangle distribution $\tri_\quant$, 
the optimal revenue is $2 - \quant$, 
and the revenue of the second price auction is $1$. 
Moreover, the quantile 
corresponding to the price of $\quant$ 
scaled up by a ratio of $\ratio \geq 1$ is 
$$\ScaledQuant(\quant, \ratio) = \frac{\quant}{\ratio - \quant\ratio + \quant}.$$
Therefore, for any $r > 1$ and $q \in [0, 1)$, 
the revenue of post price $r \cdot \vsec$
to the highest bidder is 
\begin{eqnarray*}
\Rev{\mecha_r, \tri_\quant} 
&=& 
2 \ratio 
\int_{\ScaledQuant(\quant, \sfrac{1}{\ratio})}^{1}
\valf(\quant') 
\ScaledQuant(\quant', \ratio)
\,d\quant' \\
&=& 
2 \ratio 
\int_{\ScaledQuant(\quant, \sfrac{1}{\ratio})}^{1}
\frac{1-\quant'}{1-\quant} \cdot 
\frac{1}{\ratio - \quant'\ratio + \quant'}
\,d\quant' \\
&=& 
\frac{2 \ratio}{(1-\quant)(\ratio-1)}
\int_{\ScaledQuant(\quant, \sfrac{1}{\ratio})}^{1}
\left(1- 
\frac{1}{\ratio - \quant'\ratio + \quant'}
\right)
\,d\quant' \\
&=& 
\frac{2\ratio}{(1-\quant)(\ratio-1)} 
\left(
\frac{1-\quant}{1-\quant+\quant\ratio}
+
\frac{\ln \left(
\frac{\ratio}{1-\quant+\quant\ratio}
\right)}{1-\ratio}
\right). 
\end{eqnarray*}
% \todo[inline]{Prove that $\Rev{\mecha_r, \tri_\quant}$ is quasi-concave in $r$.}

To numerically approximate the program, 
we show that the revenue changes moderately when the monopoly quantile $\quant$
and the factor $\ratio$ changes. 
\begin{claim}\label{clm:cont in r}
For any distribution $\dist$, for any $1 \leq \ratio_1 \leq \ratio_2$, 
we have $\Rev{\mecha_{\ratio_1}, \dist} \geq 
\sfrac{\ratio_1}{\ratio_2} \cdot \Rev{\mecha_{\ratio_2}, \dist}$. 
\end{claim}
\begin{proof}
For any realized valuation profile, 
if the mechanism is sold in mechanism $\mecha_{\ratio_2}$, 
then the mechanism is sold in mechanism $\mecha_{\ratio_1}$. 
Moreover, 
when the item is sold in mechanism $\mecha_{\ratio_1}$, 
the payment from agent with highest type is at least 
$\sfrac{\ratio_1}{\ratio_2}$ fraction of 
the payment in mechanism $\mecha_{\ratio_2}$. 
Taking expectation over the valuation profiles, 
we have $\Rev{\mecha_{\ratio_1}, \dist} \geq 
\sfrac{\ratio_1}{\ratio_2} \cdot \Rev{\mecha_{\ratio_2}, \dist}$. 
\end{proof}

\begin{claim}\label{clm:cont in q}
For any mechanism $\mecha_{\ratio}$ with $\ratio \geq 1$, 
and for any $\quant_1 \leq \quant_2$, 
we have 
$\Rev{\mecha_{\ratio}, \tri_{\quant_1}} \leq 
\quant_2 - \quant_1 
+ \Rev{\mecha_r, \tri_{\quant_2}}$.
\end{claim}
\begin{proof}
By directly comparing the revenue from two distributions, 
\begin{eqnarray*}
\Rev{\mecha_r, \tri_{\quant_1}} 
&=& 
2 \ratio 
\int_{\ScaledQuant(\quant_1, \sfrac{1}{\ratio})}^{1}
\valf_{\tri_{\quant_1}}(\quant') 
\ScaledQuant(\quant', \ratio)
\,d\quant' \\
&\leq& - \ScaledQuant(\quant_1, \sfrac{1}{\ratio})
+ \ScaledQuant(\quant_2, \sfrac{1}{\ratio}) 
+ \int_{\ScaledQuant(\quant_2, \sfrac{1}{\ratio})}^{1}
\valf_{\tri_{\quant_1}}(\quant') 
\ScaledQuant(\quant', \ratio)
\,d\quant' \\
&\leq& \quant_2 - \quant_1 
+ \int_{\ScaledQuant(\quant_2, \sfrac{1}{\ratio})}^{1}
\valf_{\tri_{\quant_2}}(\quant') 
\ScaledQuant(\quant', \ratio)
\,d\quant' \\
&=& 
\quant_2 - \quant_1 
+ \Rev{\mecha_r, \tri_{\quant_2}}.
\end{eqnarray*}
The second inequality holds because 
$\valf_{\tri_{\quant_1}}(\quant') \leq \valf_{\tri_{\quant_2}}(\quant') $
for $\quant_1 \leq \quant_2$ 
and $\quant' \geq \quant_2$, 
and 
$\ScaledQuant(\quant_2, \sfrac{1}{\ratio}) 
- \ScaledQuant(\quant_1, \sfrac{1}{\ratio})
\leq \quant_2 - \quant_1$. 
\end{proof}

Let $r(\quant) = \arg\max_{r>1} \Rev{\mecha_r, \tri_\quant}$. 
By solving 
\begin{align*}
\quant^* = \arg\min_\quant \quad \min\left\{2-\quant, 
\frac{2-\quant}{\Rev{\mecha_{r(\quant)}, \tri_\quant}}\right\}, 
\end{align*}
we get the desired parameters in \Cref{thm:upper}. 
Note that for distribution $\tri_\quant$ with $\quant \leq 0.05$, 
approximation ratio is larger than $1.95$, 
and for distribution $\tri_\quant$ with $\quant \geq 0.05$, 
the approximation ratio for $\ratio \geq 20$ is larger than 2. 
By \Cref{clm:cont in r} and \ref{clm:cont in q}, 
we can discretize the quantile $\quant$ and the ratio $\ratio$
to find the numerically optimal solution. 
\end{proof}



\begin{theorem}\label{thm:lower}
There exists a constant $\alpha \in [\sfrac{1}{2}, 1]$ 
such that 
for mechanism $\mecha^*$, which posts second price $\vsec$
with probability $\alpha$ 
and posts $r^* \vsec$ with probability $1-\alpha$, 
the worst case distribution is $\tri_{\quant^*}$. 
\end{theorem}

Combining \Cref{thm:upper} and \ref{thm:lower}, 
we have 
\begin{align*}
\max_{\mecha \in \scalei}
\min_{\dist \in \regular}
\frac{\OPT(\dist)}{\Rev{\mecha, \dist}} 
\geq \min_{\dist \in \tri}
\max_{\mecha \in \scalei}
\frac{\OPT(\dist)}{\Rev{\mecha, \dist}}.
\end{align*}
Also by weak duality, we have 
\begin{align*}
\max_{\mecha \in \scalei}
\min_{\dist \in \regular}
\frac{\OPT(\dist)}{\Rev{\mecha, \dist}} 
\leq \min_{\dist \in \regular}
\max_{\mecha \in \scalei}
\frac{\OPT(\dist)}{\Rev{\mecha, \dist}}
\leq \min_{\dist \in \tri}
\max_{\mecha \in \scalei}
\frac{\OPT(\dist)}{\Rev{\mecha, \dist}}.
\end{align*}
Combining the inequalities, we have
\begin{align*}
\max_{\mecha \in \scalei}
\min_{\dist \in \regular}
\frac{\OPT(\dist)}{\Rev{\mecha, \dist}} 
= \min_{\dist \in \tri}
\max_{\mecha \in \scalei}
\frac{\OPT(\dist)}{\Rev{\mecha, \dist}}
\approx 1.907.
\end{align*}
This implies that the mechanism found in \Cref{thm:upper} is optimal. 

To prove \Cref{thm:lower}, first we have the following lemma characterizing 
the worst case distribution for a family of scale invariant mechanisms. 

\begin{lemma}\label{lem:quad}
For any $\alpha \in [\sfrac{1}{2}, 1], r\geq 1$, the mechanism $\mechaAR$ that posts second highest value $\vsec$ to the highest value agent with probability $\alpha$, 
and posts $r \cdot \vsec$ to the highest value agent with probability $1-\alpha$, 
the worst case distribution is a quadrilateral distribution. 
\end{lemma}
\begin{proof}
For any distribution $\dist$ with monopoly quantile $\qo$, 
let $\qt$ be the quantile corresponds to value $\sfrac{1}{\qt r}$. 
By \Cref{...}, 
there exists a distribution $\bar{\dist}$ such that for any $\val \geq \sfrac{1}{\qo}$, 
$\bar{\dist}(\val) = 1$, 
for any $\val < \sfrac{1}{\qo}$, 
$\bar{\dist}(\val) = \dist(\val)$, 
and 
$$\frac{\OPT(\dist)}{\Rev{\mechaAR, \dist}} \leq \frac{\OPT(\bar{\dist})}{\Rev{\mechaAR, \bar{\dist}}}.$$
Note that for distribution $\bar{\dist}$, the optimal revenue $\OPT(\bar{\dist}) = 2 - \qo$, 
% Letting $\val(\quant)$ be the mapping from quantile to value 
% and $\bar{R}(\quant)$ be the mapping from quantile to the revenue of posting price $\val(\quant)$ given the distribution $\bar{\dist}$, 
and the revenue of mechanism $\mechaAR$ is  
% \begin{align*}
% \Rev{\mechaAR, \bar{\dist}} &= 
% 2\alpha \int_0^1 -\bar{R}' (\quant) \cdot (1-\bar{\dist}(\val(\quant))) \, dq
% + 2(1-\alpha) \int_0^1 -\bar{R}' (\quant) 
% \cdot \left(1-\bar{\dist}\left(\frac{\val(\quant)}{r}\right)\right) \, dq\\
% &= -\alpha\quant - 2\alpha\int_{\qo}^1 \bar{R}' (\quant) \cdot (1-\bar{\dist}(\val(\quant))) \, dq
% - .
% \end{align*}
\begin{align*}
\Rev{\mechaAR, \bar{\dist}} = 
\alpha \Rev{\mecha_1, \bar{\dist}}
+ (1-\alpha) \Rev{\mecha_r, \bar{\dist}}.
\end{align*}
We bound the revenue in two parts. 
Let $\Tilde{\dist} = \Qr_{\qo, \qt, r}$ 
be the quadrilateral distribution with quantile $\qo$ and $\qt$. 
By regularity of distribution $\bar{\dist}$, 
we have $\rev_{\bar{\dist}}(\quant) \geq \rev_{\Tilde{\dist}}(\quant)$
and $\valf_{\bar{\dist}}(\quant) \geq \valf_{\Tilde{\dist}}(\quant)$
for any $\quant\in[0, 1]$. 
Therefore, for the revenue comes from second price auction, 
\begin{align*}
\Rev{\mecha_1, \bar{\dist}} = \int_0^1 \rev_{\bar{\dist}}(\quant) \, dq
\geq \int_0^1 \rev_{\Tilde{\dist}}(\quant) \, dq
= \Rev{\mecha_1, \Tilde{\dist}}. 
\end{align*}
Let $\hat{\dist}$ 
be the distribution such that $\hat{\dist}(\quant) = \Tilde{\dist}(\quant)$ 
for any $\quant \in [0, \qt]$, 
and $\hat{\dist}(\quant) = \bar{\dist}(\quant)$
for any $\quant \in [\qt, 1]$. 
Similarly, for the revenue comes from mechanism $\mecha_r$,
\begin{align*}
\Rev{\mecha_r, \bar{\dist}} 
&= \int_0^1 r \cdot \valf_{\bar{\dist}}(\quant) (1-\bar{\dist}(r \cdot \valf_{\bar{\dist}}(\quant)))\, dq \\
&= \int_{\bar{\quant'}}^1 r \cdot \valf_{\bar{\dist}}(\quant) (1-\bar{\dist}(r \cdot \valf_{\bar{\dist}}(\quant)))\, dq \\
&\geq \int_{\bar{\quant'}}^1 r \cdot \valf_{\hat{\dist}}(\quant) (1-\hat{\dist}(r \cdot \valf_{\hat{\dist}}(\quant)))\, dq \\
&= \Rev{\mecha_r, \hat{\dist}}, 
\end{align*}
where the second inequality holds because $\bar{\dist}(r \cdot \valf_{\bar{\dist}}(\quant)) = 1$
for any $\quant < \qt$. 
The inequality holds because $\valf_{\bar{\dist}}(\quant) = \valf_{\hat{\dist}}(\quant)$ 
for $\quant \in [\qt, 1]$
and $\bar{\dist}(\val) \leq \hat{\dist}(\val)$ for any $\val$. 
Now we can rewrite the revenue $\Rev{\mecha_r, \hat{\dist}}$ and have
\begin{align*}
\Rev{\mecha_r, \hat{\dist}} 
&= \int_0^1 -\rev'_{\hat{\dist}}(\quant) \cdot \left(1-\hat{\dist}\left(
\frac{\valf_{\hat{\dist}}(\quant)}{r}\right)\right) \, dq \\
&= -\qt - \int_{\qo}^{\bar{\quant'}} 
\rev'_{\hat{\dist}}(\quant) \cdot \left(1-\hat{\dist}\left(
\frac{\valf_{\hat{\dist}}(\quant)}{r}\right)\right) \, dq
- \int_{\bar{\quant'}}^1 
\rev'_{\hat{\dist}}(\quant) \cdot \left(1-\hat{\dist}\left(
\frac{\valf_{\hat{\dist}}(\quant)}{r}\right)\right) \, dq \\
&\geq -\qt - \int_{\qo}^{\bar{\quant'}} 
\rev'_{\Tilde{\dist}}(\quant) \cdot \left(1-\hat{\dist}\left(
\frac{\valf_{\Tilde{\dist}}(\quant)}{r}\right)\right) \, dq
- \int_{\bar{\quant'}}^1 
\rev'_{\hat{\dist}}(\quant) \cdot \left(1-\hat{\dist}\left(
\frac{\valf_{\hat{\dist}}(\quant)}{r}\right)\right) \, dq \\
&\geq -\qt - \int_{\qo}^{\bar{\quant'}} 
\rev'_{\Tilde{\dist}}(\quant) \cdot \left(1-\hat{\dist}\left(
\frac{\valf_{\Tilde{\dist}}(\quant)}{r}\right)\right) \, dq \\
& \quad + \frac{\qt}{r\qo \cdot (1-\qt)^2} 
\left(1-\qt - \frac{1}{r-1} 
\cdot \ln \left(\frac{r}{1+(r-1)\qt}
\right)\right)\\
& = \Rev{\mecha_r, \Tilde{\dist}}. 
\end{align*}
The first inequality holds because 
$\rev'_{\hat{\dist}}(\quant) = \rev'_{\Tilde{\dist}}(\quant)$ 
for any $\quant\in [\qo, \qt]$, 
and $\hat{\dist}(\val) \leq \Tilde{\dist}(\val)$ for any $\val$.
The second inequality holds by proof of proposition 4 in \citet{..}. 
The last inequality holds by the definition of distribution $\Tilde{\dist}$. 
Combining the inequalities, we have
\begin{align*}
\Rev{\mechaAR, \bar{\dist}} \geq \Rev{\mechaAR, \Tilde{\dist}}.
\end{align*}
Since the optimal revenue for quadrilateral distribution $\Tilde{\dist}$
is $\OPT(\Tilde{\dist}) = 2 - \qo$ as well,
we have 
\begin{align*}
\frac{\OPT(\dist)}{\Rev{\mechaAR, \dist}} 
\leq \frac{\OPT(\bar{\dist})}{\Rev{\mechaAR, \bar{\dist}}}
\leq \frac{\OPT(\Tilde{\dist})}{\Rev{\mechaAR, \Tilde{\dist}}},
\end{align*}
which implies the worst case distribution for mechanism $\mechaAR$ is 
a quadrilateral distribution. 
\end{proof}

\begin{lemma}\label{lem:tri}
For any $\alpha \in [\sfrac{1}{2}, 1]$ and $r \in []$, 
the mechanism $\mechaAR$ that posts second highest value $\vsec$ to the highest value agent with probability $\alpha$, 
and posts $r \cdot \vsec$ to the highest value agent with probability $1-\alpha$, 
the worst case distribution when the monopoly quantile is $\qo \in [0, ]$ is a triangle distribution. 
\end{lemma}
\begin{proof}
By \Cref{lem:quad}, without loss of generality, 
we can consider the worst case distribution as a quadrilateral distribution $\Qr_{\qo, \qt, r}$. 
% The optimal revenue for distribution $\Qr_{\qo, \qt, r}$
% is $2 - \qo$,
For simplicity, we introduce the notation $\revq(\val)$
to denote the revenue of posting price $\val$,
and $\valq(\quant)$ to denote the price $\val$ given quantile $\quant$ when the distribution is $\Qr_{\qo, \qt, r}$. 
Let $\quant^*$ be the quantile such that $r \cdot \valq(\quant^*) = \sfrac{\qt}{r\cdot \qo}$.
By construction of distribution $\Qr_{\qo, \qt, r}$, we have 
$$\quant^* = \frac{r\cdot \qt}{1+(r-1)\qt}.$$
Thus, the revenue of mechanism $\mechaAR$ given distribution $\Qr_{\qo, \qt, r}$ is as follows.  For sub-calculations substituted into this sequence, see below.
\begin{align*}
\Rev{\mechaAR, \Qr_{\qo, \qt, r}}
&= 
\alpha \Rev{\mecha_1, \Qr_{\qo, \qt, r}}
+ (1-\alpha) \Rev{\mecha_r, \Qr_{\qo, \qt, r}} \\
&= 2\alpha \int_0^1 \rev_{\Qr_{\qo, \qt, r}}(q) \, dq
+ 2(1-\alpha) \int_0^1 \revq(r\cdot \valq(\quant)) \, dq \\
&= \alpha \left(\qo + (\qt - \qo)(1+\frac{\qt}{r\cdot \qo}) + (1-\qt)\frac{\qt}{r\cdot \qo}\right) \\
& \quad + 2(1-\alpha)\int_{\qt}^{\quant^*} \rev_{\Qr_{\qo, \qt, r}}(q) \, dq
+ 2(1-\alpha)\int_{\quant^*}^1 \rev_{\Qr_{\qo, \qt, r}}(q) \, dq \\
&= \alpha \left(\qo + (\qt - \qo)(1+\frac{\qt}{r\cdot \qo}) + (1-\qt)\frac{\qt}{r\cdot \qo}\right) \\
& \quad + 2(1-\alpha)\int_{\qt}^{\quant^*} \left(\frac{\qt(1-\qt)(\qo r-\qo)}{(\qt-\qo)r \qt (1-q)+q(1-\qt)(\qo r -\qt)} 
\right) \cdot \frac{\qt}{\qo}\cdot \frac{1-q}{1-\qt}\, dq \\
& \quad + 2(1-\alpha)\int_{\quant^*}^1 \frac{1}{r-(r-1)q}\cdot\frac{\qt}{\qo}\cdot\frac{1-q}{1-\qt} \, dq\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\int_{\qt}^{\quant^*} \left(\frac{1-q}{(\qt-\qo)r \qt +q(\qo r-\qt-(r-1)\qt^2)} \right)\, dq \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\int_{\quant^*}^1 \frac{1-q}{r-(r-1)q} \, dq\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-q}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln((\qt-\qo)r \qt +q(\qo r-\qt-(r-1)\qt^2) )}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right]_{\qt}^{\quant^*} \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{q}{r-1}+\frac{\ln(r-(r-1)q)}{(r-1)^2} \right]_{\quant^*}^1\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-(\quant^*-\qt)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{(\qt-\qo)r \qt +\quant^*(\qo r-\qt-(r-1)\qt^2)}{(\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right] \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\quant^*}{r-1}-\frac{\ln(r-(r-1)\quant^*)}{(r-1)^2} \right]
\end{align*}

\noindent We substitute out $\quant^*$.

\begin{align*}
    1-\quant^* &= \frac{1-\qt}{1+(r-1)\qt}\\
    r-(r-1)\quant^* &= \frac{r(1+(r-1)\qt)}{1+(r-1)\qt}-\frac{(r-1)(1-\qt)}{1+(r-1)\qt} =\frac{r+r(r-1)\qt -r+r\qt +1-\qt}{1+(r-1)\qt}=\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt}\\
&\quad \Rev{\mechaAR, \Qr_{\qo, \qt, r}}\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qt\cdot((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}{((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right] \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\qt}{(r-1)(1+(r-1)\qt)}-\frac{\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)}{(r-1)^2} \right]
\end{align*}

\noindent We handle each derivative of the additive terms.

\begin{align*}
    & \quad \partial \left(\alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right)  \right) / \partial \qt =  \alpha\left(1 + \frac{1-\qo}{\qo r}\right)\\
    %1-\quant^* &= \frac{1-\qt}{1+(r-1)\qt}\\
    %r-(r-1)\quant^* &= \frac{r(1+(r-1)\qt)}{1+(r-1)\qt}-\frac{(r-1)(1-\qt)}{1+(r-1)\qt} =\frac{r+r(r-1)\qt -r+r\qt +1-\qt}{1+(r-1)\qt}=\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt}\\
    & \quad \partial \left( 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\qt}{(r-1)(1+(r-1)\qt)}-\frac{\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)}{(r-1)^2} \right]\right) /\partial \qt\\
    = & \quad \partial \left( 2(1-\alpha)\cdot \left[
\frac{\qt}{\qo(r-1)(1+(r-1)\qt)}-\frac{\qt\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)}{\qo(1-\qt)(r-1)^2} \right]\right) /\partial \qt\\
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)}{q(r-1)^2}\cdot\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
    &\quad -\frac{2(1-\alpha)\qt}{q(r-1)^2(1-\qt)}\cdot\left[\frac{r^2-1}{r^2\qt+(1-\qt)}-\frac{r-1}{1+(r-1)\qt} \right]\\
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)^2}\right)\cdot\frac{r-1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)}{q(r-1)^2}\cdot\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
    &\quad -\frac{2(1-\alpha)\qt}{q(r-1)^2(1-\qt)}\cdot\left[\frac{r(r-1)}{(r^2\qt+(1-\qt))(1+(r-1)\qt)}\right]\\
    \geq & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)^2}\right)\cdot\frac{r-1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)}{q(r-1)^2}\cdot\frac{1}{(1-\qt)^2}\\
    &\quad -\frac{2(1-\alpha)\qt}{q(r-1)^2(1-\qt)}\cdot\left[\frac{r(r-1)}{(r^2\qt+(1-\qt))(1+(r-1)\qt)}\right]\\
\intertext{by $\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)\leq \ln\left(\frac{r^2\qt+r(1-\qt)}{1+(r-1)\qt} \right)= \ln r \leq 1$, assuming $1\leq r \leq \exp(1)$; however, perhaps another substitution using the Taylor Series approximation bounds on $\ln$-function is more appropriate}
    %= & \frac{2(1-\alpha)}{\qo}\cdot\frac{(r-1)(1-\qt)^2(r^2\qt+(1-\qt))-(r^2\qt+(1-\qt))(1+(r-1)\qt)^2 }{(r-1)^2(1-\qt)^2(r^2\qt+(1-\qt)(1+(r-1)\qt)^2}\\
    %& \quad + \frac{2(1-\alpha)}{\qo}\cdot\frac{-(r-1)(1-\qt)(1+(r-1)\qt)r}{(r-1)^2(1-\qt)^2(r^2\qt+(1-\qt)(1+(r-1)\qt)^2}
\end{align*}

\begin{align*}
    & \quad \partial \left(2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.
    \right.\\
    &\quad \left. \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qt\cdot((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}{((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right]\right)/\partial \qt\\
    =& \quad \left(2(1-\alpha)\frac{2\qt(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.
    \right.\\
    &\quad \left. \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qt\cdot((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}{((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right]\right)\\
    &\quad +\left(2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{+\left( \frac{(r-1)(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot (-1-2(r-1)\qt)\right.\right.
    \right.\\
    &\quad +\frac{+\left( \frac{(r-1)(1-\qt)}{(1+(r-1)\qt)^2}\cdot(r-1)\right)}{(\qo r-\qt-(r-1)\qt^2)}+\frac{+\left( \frac{(r-1)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\\
    &\quad +\frac{\left(-1\cdot((\qo r-\qt)+(1-\qt))\right)\cdot \ln\left(\frac{r \qt\cdot((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}{((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2}\\
    &\quad +\frac{-2\cdot\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qt\cdot((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}{((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^3\cdot(-1-2(r-1)\qt )^{-1}}\\
    &\quad +\frac{\left((\qo r-\qt)(1-\qt)\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot\left(\frac{1}{\qt}+\frac{(1+(r-1)\qt+(r-1)(\qt-\qo))+(-1-2(r-1)\qt) }{((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}\right) \\
    &\quad -\frac{\left((\qo r-\qt)(1-\qt)\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot\frac{r(\qt-\qo)+r\qt+(\qo r-\qt-(r-1)\qt^2) +\qt(-1-2(r-1)\qt)} {((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))}\\
    &\quad \left. \left.\left.-\frac{\left((\qo r-\qt)(1-\qt)\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot\frac{r-1} {(1+(r-1)\qt)} \right]\right]\right)\end{align*}

\end{proof}

\noindent\textbf{The following gives sub-calculations in support of the preceding.}

\noindent We give the identity for $\quant^*$.  We can calculate the height of the quadrilateral revenue curve at $\quant^*\in[\qt,1]$ from two formulas each using $\quant^*$.  We can set them equal and solve.
\begin{align}
    \text{height at}~\quant^*\in[\qt,1]:\quad \quant^*\cdot\frac{1}{\qo r^2} &= \frac{\qt}{\qo r}\cdot\frac{1-\quant^*}{1-\qt}\\
    \quant^*(1-\qt) &= r \qt(1-\quant^*)\\
    \quant^*(1-\qt) &= r\qt-r\qt \quant^*\\
    \quant^*\left((1-\qt)+r \qt \right) &= r\qt\\
    \quant^* &= \frac{\qt r}{(1-\qt)+\qt r} = \frac{\qt r}{1+(r-1)\qt}
\intertext{we note this also induces for substitution:}
    1-\quant^* &= \frac{1-\qt}{1+(r-1)\qt}\\
    r - (r-1)\quant^* &= \frac{r(1+(r-1)\qt)}{1+(r-1)\qt}-\frac{(r-1)(1-\qt)}{1+(r-1)\qt}\\
    &= \frac{r + r(r-1)\qt-r+r\qt+1-\qt}{1+(r-1)\qt} = \frac{r^2\qt +(1-\qt)}{1+(r-1)\qt}
\end{align}

\noindent Given the quadrilateral curve, the value $v^*$ associated with quantile $q\in[\quant^*,1]$, and the value $v'$ for $q\in[\qt,\quant^*]$, are
\begin{align}
    v^*(q) &= \frac{1}{q}\cdot\left(\frac{1-q}{1-\qt}\right)\cdot\frac{\qt}{\qo r}\\
    v'(q) &= \left(\frac{\qt-\quant^*}{\qt-\qo}\right)\left(1-\frac{\qt}{\qo r}\right)+\frac{\qt}{\qo r}
\intertext{A price scaled up by a factor of $r$ given $q\in[\qt,1]$ is}
    r\cdot v^*(q) &= \frac{\qt}{\qo q}\cdot\left(\frac{1-q}{1-\qt}\right)
\end{align}

\noindent The following {\em does not} condition the ``probability of sale" to try to sell to an agent with quantile smaller than the input $q$; this quantity follows from the ending calculated terms, divided by $q$.  The probability of sale $k$ given $q\in[\qt,\quant^*]$ and corresponding value as price scaled up by $r$ can be found from the intersection of
\begin{align}
    \frac{\qt}{\qo q}\left(\frac{1-q}{1-\qt}\right)k & = \left(\frac{\qt-\quant^*}{\qt-\qo}\right)\left(1-\frac{\qt}{\qo r}\right) + \frac{\qt}{\qo r}\\
    (\qt-\qo)\frac{r\qt}{q}(1-q)k &= (\qt-\quant^*)(1-\qt)(\qo r-\qt)+\qt(\qt-\qo)(1-\qt)\\
    \left[(\qt-\qo)\frac{r\qt}{q}(1-q)+(1-\qt)(\qo r-\qt) \right]k &= \qt(1-\qt)(\qo r - \qo)\\
    k&= \frac{q\qt(1-\qt)(\qo r-\qo)}{(\qt-\qo)r\qt(1-q)+q(1-\qt)(\qo r-\qt)}
\end{align}

\noindent Finally with similar technique, we determine the probability of sale for the scale-up price given $q\in[\quant^*,1]$:

\begin{align}
    \frac{\qt}{\qo q}\left(\frac{1-q}{1-\qt}\right)k &= \left(\frac{1-\quant^*}{1-\qt}\right)\cdot\frac{\qt}{\qo r}\\
    r(1-q)k&= (1-\quant^*)q\\
    k&= \frac{q}{r-(r-1)q}
\end{align}






\begin{proof}[Proof of \Cref{thm:upper}]
By \Cref{lem:tri}, for $\alpha \in [0.8, 0.81]$ and $r \in [2.44, 2.45]$, 
the mechanism $\mechaAR$ that posts second highest value $\vsec$ to the highest value agent with probability $\alpha$, 
and posts $r \cdot \vsec$ to the highest value agent with probability $1-\alpha$, 
the worst case distribution when the monopoly quantile is $\qo \in [0, ]$ is a triangle distribution. 



By numerical computation, for $r \in [2.44, 2.45]$, 
when $\alpha = 0.81$, the worst case distribution for mechanism $\mechaAR$
is triangle distribution with monopoly quantile at most $0.087$, 
and when $\alpha = 0.8$, the worst case distribution for mechanism $\mechaAR$
is triangle distribution with monopoly quantile at least $0.101$. 
By continuity of the program, there for $\ratio^* \approx 2.446946$, 
there exists $\alpha^*$ such that the worst case distribution 
is triangle distribution with monopoly quantile $\quant^* \approx 0.0931057$. 
By numerical computation, we have $\alpha^* \approx 0.8056405$. 
\end{proof}

==> old-files/monotone-old.tex <==
\begin{lemma}\label{lem:tri}
For revenue maximization with 2 agents, 
and for any $\alpha \in [\sfrac{2}{3}, 1]$ and $r \geq 1$, 
the mechanism $\mechaAR$ that posts second highest value $\vsec$ to the highest value agent with probability $\alpha$, 
and posts $r \cdot \vsec$ to the highest value agent with probability $1-\alpha$, 
the worst case distribution is a triangle distribution. 
\end{lemma}
\begin{proof}
By \Cref{lem:quad}, without loss of generality, 
we can consider the worst case distribution as a quadrilateral distribution $\Qr_{\qo, \qt, \ratio}$. 
% The optimal revenue for distribution $\Qr_{\qo, \qt, \ratio}$
% is $2 - \qo$,
For simplicity, we introduce the notation $\revq(\val)$
to denote the revenue of posting price $\val$,
and $\valq(\quant)$ to denote the price $\val$ given quantile $\quant$ when the distribution is $\Qr_{\qo, \qt, \ratio}$. 
Let $\quant^*$ be the quantile such that $r \cdot \valq(\quant^*) = \sfrac{\qt}{r\cdot \qo}$.
By construction of distribution $\Qr_{\qo, \qt, \ratio}$, we have 
$$\quant^* = \frac{r\cdot \qt}{1+(r-1)\qt}.$$
Thus, the revenue of mechanism $\mechaAR$ given distribution $\Qr_{\qo, \qt, \ratio}$ is as follows.  For sub-calculations substituted into this sequence, see below.
\begin{align}
\Rev{\mechaAR, \Qr_{\qo, \qt, \ratio}}
&= 
\alpha \Rev{\mecha_1, \Qr_{\qo, \qt, \ratio}}
+ (1-\alpha) \Rev{\mecha_r, \Qr_{\qo, \qt, \ratio}} \\
&= 2\alpha \int_0^1 \rev_{\Qr_{\qo, \qt, \ratio}}(q) \, dq
+ 2(1-\alpha) \int_0^1 \revq(r\cdot \valq(\quant)) \, dq \\
&= \alpha \left(\qo + (\qt - \qo)(1+\frac{\qt}{r\cdot \qo}) + (1-\qt)\frac{\qt}{r\cdot \qo}\right) \\
& \quad + 2(1-\alpha)\int_{\qt}^{\quant^*} \rev_{\Qr_{\qo, \qt, \ratio}}(q) \, dq
+ 2(1-\alpha)\int_{\quant^*}^1 \rev_{\Qr_{\qo, \qt, \ratio}}(q) \, dq \\
&= \alpha \left(\qo + (\qt - \qo)(1+\frac{\qt}{r\cdot \qo}) + (1-\qt)\frac{\qt}{r\cdot \qo}\right) \\
& \quad + 2(1-\alpha)\int_{\qt}^{\quant^*} \left(\frac{\qt(1-\qt)(\qo r-\qo)}{(\qt-\qo)r \qt (1-q)+q(1-\qt)(\qo r -\qt)} 
\right) \cdot \frac{\qt}{\qo}\cdot \frac{1-q}{1-\qt}\, dq \\
& \quad + 2(1-\alpha)\int_{\quant^*}^1 \frac{1}{r-(r-1)q}\cdot\frac{\qt}{\qo}\cdot\frac{1-q}{1-\qt} \, dq\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\int_{\qt}^{\quant^*} \left(\frac{1-q}{(\qt-\qo)r \qt +q(\qo r-\qt-(r-1)\qt^2)} \right)\, dq \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\int_{\quant^*}^1 \frac{1-q}{r-(r-1)q} \, dq\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-q}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln((\qt-\qo)r \qt +q(\qo r-\qt-(r-1)\qt^2) )}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right]_{\qt}^{\quant^*} \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{q}{r-1}+\frac{\ln(r-(r-1)q)}{(r-1)^2} \right]_{\quant^*}^1\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
\label{eqn:condrevqtqstar1}
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-(\quant^*-\qt)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
\label{eqn:condrevqtqstar2}
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{(\qt-\qo)r \qt +\quant^*(\qo r-\qt-(r-1)\qt^2)}{(\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right] \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\quant^*}{r-1}-\frac{\ln(r-(r-1)\quant^*)}{(r-1)^2} \right]
\end{align}

\begin{lemma}
\label{lem:condrevpos}
As a function, the quantity $h(\qt)=(\qo r-\qt-(r-1)\qt^2)$ appears in line~\eqref{eqn:condrevqtqstar1} and line~\eqref{eqn:condrevqtqstar2} in the interim revenue calculation of the quadrilateral distribution. $h(\qt)<0$ for all possible values of $\qt$.  Line~\eqref{eqn:condrevqtqstar1} is a positive term and line~\eqref{eqn:condrevqtqstar2} is a negative term (both weakly).
\end{lemma}
\begin{proof}
We give an indirect proof, ultimately by contradiction.  The range of values of $\qt$ are upperbounded by $\qt_{\max}=\qo r$.  This follows by noting that- by the description of its design- the quadrilateral distribution goes through the point $(\qt, \frac{\qt}{\qo r})$ in the revenue curve graph.  We have normalized the peak revenue of the quadrilateral distribution to be 1, so this height of the revenue curve $\qt/(\qo r)\leq 1$.

By inspection, $h(\qt_{\max})=(\qo r-\qt_{\max}-(r-1)\qt^2_{\max}) = 0-(r-1)\qt^2\leq 0$.  Further, $h(\qt)$ is continuous, and it is in the denominator of line~\eqref{eqn:condrevqtqstar1}.  If $h(\qt)$ had positive output anywhere for valid inputs of $\qt$, then by continuity, the output ``moved" from negative at the maximum input $\qt_{\max}$ through 0 to positive as $\qt$ decreases in its feasible range.  Somewhere in this critical range of $\qt$, evaluation of line~\eqref{eqn:condrevqtqstar2} would go to negative infinity.  But line~\eqref{eqn:condrevqtqstar1} and line~\eqref{eqn:condrevqtqstar2} together are the revenue component when $q_{\{2\}}$ is in the range $[\qt, \quant^*]$ and the mechanism uses $r\cdot v_{\{2\}}$ as its random price.  This quantity is positive and finite, contradicting the possibility that the evaluation of~\eqref{eqn:condrevqtqstar1} is negative infinity.

Line~\eqref{eqn:condrevqtqstar2} is negative because the $\ln$ term is negative because: $\quant^*\geq \qt$ and from the above, $h(\qt)$ is negative.
\end{proof}

\noindent We substitute out $\quant^*=r\qt / (1+(r-1)\qt)$.

\begin{align}
    1-\quant^* &= \frac{1-\qt}{1+(r-1)\qt}\\
    r-(r-1)\quant^* &= \frac{r+r(r-1)\qt}{1+(r-1)\qt}-\frac{(r-1)r\qt}{1+(r-1)\qt} =\frac{r}{1+(r-1)\qt}\\
\quant^*-\qt &= \frac{r\qt}{1+(r-1)\qt}-\frac{\qt+(r-1)\qt^2}{1+(r-1)\qt} = \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\\
&\quad \Rev{\mechaAR, \Qr_{\qo, \qt, \ratio}}\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qt\cdot((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}{((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right] \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\qt}{(r-1)(1+(r-1)\qt)}-\frac{\ln\left(\frac{r}{1+(r-1)\qt} \right)}{(r-1)^2} \right]\\
\intertext{(we replace the third line using \Cref{cal:simpmonst} below)}
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right] \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\qt}{(r-1)(1+(r-1)\qt)}-\frac{\ln\left(\frac{r}{1+(r-1)\qt} \right)}{(r-1)^2} \right]
\end{align}

\begin{calc}
\label{cal:simpmonst}
\begin{align*}
& \quad  \frac{r \qt\cdot((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}{((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))\cdot(1+(r-1)\qt)}   \\
= &\quad \frac{r \qt\cdot((-\qo)(1+(r-1)\qt) +\qo r)}{(r\qt^2-\qt^2-(r-1)\qt^3)\cdot(1+(r-1)\qt)} \\
= &\quad \frac{r \qt\cdot(\qo(r-1)(1-\qt))}{(\qt^2(r-1)(1-\qt))\cdot(1+(r-1)\qt)} =  \frac{r \qo}{\qt\cdot(1+(r-1)\qt)}  \quad \bullet
\end{align*}
\end{calc}

\noindent We handle each derivative of the additive terms before combining.  The end of the calculation for each additive term is market with $\bullet$.

\begin{align}
    & \quad \partial \left(\alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right)  \right) / \partial \qt =  \alpha\left(1 + \frac{1-\qo}{r\qo}\right)=\alpha\left(\frac{1+(r-1)\qo } { r\qo} \right)\quad \bullet\\
    %1-\quant^* &= \frac{1-\qt}{1+(r-1)\qt}\\
    %r-(r-1)\quant^* &= \frac{r(1+(r-1)\qt)}{1+(r-1)\qt}-\frac{(r-1)(1-\qt)}{1+(r-1)\qt} =\frac{r+r(r-1)\qt -r+r\qt +1-\qt}{1+(r-1)\qt}=\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt}\\
    & \quad \partial \left( 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\qt}{(r-1)(1+(r-1)\qt)}-\frac{\ln\left(\frac{r}{1+(r-1)\qt} \right)}{(r-1)^2} \right]\right) /\partial \qt\\
\intertext{(multiply the $\qt/(\qo(1-\qt)$ term into the brackets)}
    = & \quad \partial \left( 2(1-\alpha)\cdot \left[
\frac{\qt}{\qo(r-1)(1+(r-1)\qt)}-\frac{\qt\ln\left(\frac{r}{1+(r-1)\qt} \right)}{\qo(1-\qt)(r-1)^2} \right]\right) /\partial \qt\\
\intertext{(evaluate the partial derivative)}
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)\qt}{\qo(r-1)^2(1-\qt)}\cdot\left[0-\frac{r-1}{1+(r-1)\qt} \right]\\
    &\quad -\frac{2(1-\alpha)}{\qo(r-1)^2}\cdot\ln\left(\frac{r}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
\intertext{(add and subtract 1 inside the $\ln$)}
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}+\frac{2(1-\alpha)\qt}{\qo(r-1)(1-\qt)}\cdot\left[\frac{1}{1+(r-1)\qt} \right]\\
    &\quad -\frac{2(1-\alpha)}{\qo(r-1)^2}\cdot\ln\left(1+\frac{r-1-(r-1)\qt}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
\intertext{(use the bound $-\ln(1+x)\geq -x$ for all $x>-1$, and in particular for $[r/ (1+(r-1)\qt)-1]\geq 0$ because the denominator is a convex combination of 1 and $r\geq 1$)}
    \geq & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}+\frac{2(1-\alpha)\qt}{\qo(r-1)(1-\qt)}\cdot\left[\frac{1}{1+(r-1)\qt} \right]\\
    &\quad -\frac{2(1-\alpha)}{\qo(r-1)^2}\cdot\left(\frac{(r-1)(1-\qt)}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
\intertext{(cancel $(r-1)(1-\qt)$) in the third term}
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}+\frac{2(1-\alpha)\qt}{\qo(r-1)(1-\qt)}\cdot\left[\frac{1}{1+(r-1)\qt} \right]\\
    &\quad -\frac{2(1-\alpha)}{\qo(r-1)}\cdot\left(\frac{1}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)}\\
\intertext{(combine the last two additive terms and then cancel $(1-\qt)$)}
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)}{\qo(r-1)}\cdot\left[\frac{1}{1+(r-1)\qt} \right]\\
\intertext{(multiply second term top-and-bottom by $(1+(r-1)\qt)$ and do final simplification)}
    = & \quad -\left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{(r-1)\qt}{(1+(r-1)\qt)^2}= -\left(\frac{2(1-\alpha)}{\qo}\right)\cdot\frac{\qt}{(1+(r-1)\qt)^2}\quad \bullet
%    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)^2}\right)\cdot\frac{r-1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)}{q(r-1)^2}\cdot\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
%    &\quad -\frac{2(1-\alpha)\qt}{q(r-1)^2(1-\qt)}\cdot\left[\frac{r(r-1)}{(r^2\qt+(1-\qt))(1+(r-1)\qt)}\right]\\
%    \geq & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)^2}\right)\cdot\frac{r-1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)}{q(r-1)^2}\cdot\frac{1}{(1-\qt)^2}\\
%    &\quad -\frac{2(1-\alpha)\qt}{q(r-1)^2(1-\qt)}\cdot\left[\frac{r(r-1)}{(r^2\qt+(1-\qt))(1+(r-1)\qt)}\right]\\
%\intertext{by $\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)\leq \ln\left(\frac{r^2\qt+r(1-\qt)}{1+(r-1)\qt} \right)= \ln r \leq 1$, assuming $1\leq r \leq \exp(1)$; however, perhaps another substitution using the Taylor Series approximation bounds on $\ln$-function is more appropriate}
    %= & \frac{2(1-\alpha)}{\qo}\cdot\frac{(r-1)(1-\qt)^2(r^2\qt+(1-\qt))-(r^2\qt+(1-\qt))(1+(r-1)\qt)^2 }{(r-1)^2(1-\qt)^2(r^2\qt+(1-\qt)(1+(r-1)\qt)^2}\\
    %& \quad + \frac{2(1-\alpha)}{\qo}\cdot\frac{-(r-1)(1-\qt)(1+(r-1)\qt)r}{(r-1)^2(1-\qt)^2(r^2\qt+(1-\qt)(1+(r-1)\qt)^2}
\end{align}

\begin{align}
    & \quad \partial \left(2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.
    \right.\\
    &\quad \left. \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right]\right)/\partial \qt\\
\intertext{(take the partial derivative which- with various applications of product rule and chain rule- requires the next 7 lines)}
    =& \quad \left(2(1-\alpha)\frac{2\qt(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.
    \right.\\
    &\quad \left. \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right]\right)\\
    &\quad +\left(2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{+\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot (-1-2(r-1)\qt)\right.\right.
    \right.\\
    &\quad +\frac{+\left( \frac{(r-1)\qt(1-\qt)}{(1+(r-1)\qt)^2}\cdot(r-1)\right)}{(\qo r-\qt-(r-1)\qt^2)}+\frac{-\left( \frac{(r-1)(1-2\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\\
    &\quad +\frac{\left(-1\cdot((\qo r-\qt)+(1-\qt))\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2}\\
    &\quad +\frac{-2\cdot\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^3}\cdot(-1-2(r-1)\qt )\\
    &\quad \left.\left.\left.-\frac{\left((\qo r-\qt)(1-\qt)\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot\left(\frac{1+2(r-1)\qt} {\qt(1+(r-1)\qt)}\right)\right]\right]\right)
\intertext{(we consolidate all lines with $\ln$ terms using \Cref{cal:consln}, which includes using the respective $2\qt$ and $\qt^2$ factors outside the brackets)}
    \geq& \quad \left(2(1-\alpha)\frac{2\qt(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right]\right]\right)\\
    &\quad +\left(2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{+\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot (-1-2(r-1)\qt)\right.\right.
    \right.\\
    &\quad +\frac{+\left( \frac{(r-1)\qt(1-\qt)}{(1+(r-1)\qt)^2}\cdot(r-1)\right)}{(\qo r-\qt-(r-1)\qt^2)}+\frac{-\left( \frac{(r-1)(1-2\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\\
    &\quad \left.\left.\left.-\frac{\left((\qo r-\qt)(1-\qt)\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot\left(\frac{1+2(r-1)\qt} {\qt(1+(r-1)\qt)}\right)\right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{\ln\left(\frac{r\qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(expand the first four lines to re-organize with common denominator, in order, again absorbing the $2\qt$ and $\qt^2$ factors outside the brackets; note that the term with factor $(1-2\qt)$ is split into two terms using $((1-\qt)-\qt)$ to simplify the next step)}%; add and subtract 1 within the $\ln$ term at the end)}
    = &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{1}{(\qo r-\qt -(r-1)\qt^2)^2(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -2\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.
    \\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)^2(1-\qt)+ \qt^3(r-1)(1+(r-1)\qt)\\
    &\quad - \qt^2(r-1)(1-\qt)(1+(r-1)\qt)\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{\ln\left(\frac{r\qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(combine some terms)}
    = &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{1}{(\qo r-\qt -(r-1)\qt^2)^2(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -3\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.
    \\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)r\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{\ln\left(\frac{r\qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(we now work towards relaxing the $\ln$ term by add-and-subtract 1 inside of it, and multiplying top-and-bottom by $(-1)$; this makes the denominator positive (as by \Cref{lem:condrevpos} the quantity $(\qo r-\qt-(r-1)\qt^2)^3$ is negative); which sets us up to lower bound a $-\ln(\cdot)$ term)}
    = &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{1}{(\qo r-\qt -(r-1)\qt^2)^2(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -3\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.
    \\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)r\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{-\ln\left(1+\frac{r\qo-\qt\cdot(1+(r-1)\qt)}{\qt\cdot(1+(r-1)\qt)} \right)}{-(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(we use the relaxation $-\ln(1+x)\geq -x$, which we can do if the rest of the factors combine to be positive, which they do: the denominator term $-(\qo r-\qt-(r-1)\qt^2)$ is positive by \Cref{lem:condrevpos} and the triple-brackets term is argued to be positive where it is derived in \Cref{cal:consln}; conveniently, the term composed of the last three lines started positive and will remain positive below)}
    \geq &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{1}{(\qo r-\qt -(r-1)\qt^2)^2(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -3\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.
    \\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)r\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{-\left(\frac{r\qo-\qt\cdot(1+(r-1)\qt)}{\qt\cdot(1+(r-1)\qt)}\right)}{-(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(in preparation to combine, multiply the first term (the first five lines) top-and-bottom by $-1(\qo r-\qt-(r-1)\qt^2)$; multiply the second term (last three lines) top-and-bottom by $(1+(r-1)\qt)^2$ and cancel a factor top-and-bottom of $\qt$)}
    \geq &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{-(\qo r-\qt-(r-1)\qt^2)}{(-(\qo r-\qt -(r-1)\qt^2)^3)(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -3\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.\\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)r\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{(\qt\cdot(1+(r-1)\qt)- r \qo)(1+(r-1)\qt)}{(-(\qo r-\qt-(r-1)\qt^2)^3)(1+(r-1)\qt)^2 } \right)\cdot\\
    &\quad [[[(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^3(\qo r-\qt)(r-1)+\qt^3(1-\qt)(r-1)]]]
\end{align}

\end{proof}

\begin{calc}
\label{cal:consln}
\begin{align*}
    &\quad +2\qt(\qo r-\qt)(1-\qt)((\qo r-\qt)-(r-1)\qt^2)\\
    &\quad + 2\qt^2(\qo r-\qt)(1-\qt)(1+2(r-1)\qt)\\
    &\quad - \qt^2((\qo r-\qt)+(1-\qt))((\qo r-\qt)-(r-1)\qt^2)\\
    = & \quad 2\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+(r-1)\qt^2\right]\\
    &\quad - \qt^2(\qo r-\qt)((\qo r-\qt)-(r-1)\qt^2)-\qt^2(1-\qt)((\qo r-\qt)-(r-1)\qt^2)\geq0\\
\intertext{{\em (where the inequality follows because the positive term (first row) has all positive factors, and each ``negative" term (second row) has a factor of $(\qo r-\qt)-(r-1)\qt^2)<0$ by \Cref{lem:condrevpos}, such that they are actually positive; we continue manipulation to further simplify substitution into the main calculation of the derivative)}}
    \Leftrightarrow & \quad \qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-\qt)\\
    &\quad - \qt^2(\qo r-\qt)((\qo r-\qt)-(r-1)\qt^2)+\qt^4(1-\qt)(r-1)\geq 0\\
    \Leftrightarrow & \quad \qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)\geq 0 \quad \bullet
\intertext{{\em (where each further manipulation has been re-arrangement of the left-hand side with equality such that it is necessarily still non-negative overall; however, the third term individually is possibly negative due to the $(1-2\qt)$ term)}}
\end{align*}
\end{calc}



\noindent\textbf{The following gives sub-calculations in support of the preceding.}

\noindent We give the identity for $\quant^*$.  We can calculate the height of the quadrilateral revenue curve at $\quant^*\in[\qt,1]$ from two formulas each using $\quant^*$.  We can set them equal and solve.
\begin{align}
    \text{height at}~\quant^*\in[\qt,1]:\quad \quant^*\cdot\frac{1}{\qo r^2} &= \frac{\qt}{\qo r}\cdot\frac{1-\quant^*}{1-\qt}\\
    \quant^*(1-\qt) &= r \qt(1-\quant^*)\\
    \quant^*(1-\qt) &= r\qt-r\qt \quant^*\\
    \quant^*\left((1-\qt)+r \qt \right) &= r\qt\\
    \quant^* &= \frac{\qt r}{(1-\qt)+\qt r} = \frac{\qt r}{1+(r-1)\qt}
\intertext{we note this also induces for substitution:}
    1-\quant^* &= \frac{1-\qt}{1+(r-1)\qt}\\
    r - (r-1)\quant^* &= \frac{r(1+(r-1)\qt)}{1+(r-1)\qt}-\frac{(r-1)(1-\qt)}{1+(r-1)\qt}\\
    &= \frac{r + r(r-1)\qt-r+r\qt+1-\qt}{1+(r-1)\qt} = \frac{r^2\qt +(1-\qt)}{1+(r-1)\qt}
\end{align}

\noindent Given the quadrilateral curve, the value $v^*$ associated with quantile $q\in[\quant^*,1]$, and the value $v'$ for $q\in[\qt,\quant^*]$, are
\begin{align}
    v^*(q) &= \frac{1}{q}\cdot\left(\frac{1-q}{1-\qt}\right)\cdot\frac{\qt}{\qo r}\\
    v'(q) &= \left(\frac{\qt-\quant^*}{\qt-\qo}\right)\left(1-\frac{\qt}{\qo r}\right)+\frac{\qt}{\qo r}
\intertext{A price scaled up by a factor of $r$ given $q\in[\qt,1]$ is}
    r\cdot v^*(q) &= \frac{\qt}{\qo q}\cdot\left(\frac{1-q}{1-\qt}\right)
\end{align}

\noindent The following {\em does not} condition the ``probability of sale" to try to sell to an agent with quantile smaller than the input $q$; this quantity follows from the ending calculated terms, divided by $q$.  The probability of sale $k$ given $q\in[\qt,\quant^*]$ and corresponding value as price scaled up by $r$ can be found from the intersection of
\begin{align}
    \frac{\qt}{\qo q}\left(\frac{1-q}{1-\qt}\right)k & = \left(\frac{\qt-\quant^*}{\qt-\qo}\right)\left(1-\frac{\qt}{\qo r}\right) + \frac{\qt}{\qo r}\\
    (\qt-\qo)\frac{r\qt}{q}(1-q)k &= (\qt-\quant^*)(1-\qt)(\qo r-\qt)+\qt(\qt-\qo)(1-\qt)\\
    \left[(\qt-\qo)\frac{r\qt}{q}(1-q)+(1-\qt)(\qo r-\qt) \right]k &= \qt(1-\qt)(\qo r - \qo)\\
    k&= \frac{q\qt(1-\qt)(\qo r-\qo)}{(\qt-\qo)r\qt(1-q)+q(1-\qt)(\qo r-\qt)}
\end{align}

\noindent Finally with similar technique, we determine the probability of sale for the scale-up price given $q\in[\quant^*,1]$:

\begin{align}
    \frac{\qt}{\qo q}\left(\frac{1-q}{1-\qt}\right)k &= \left(\frac{1-\quant^*}{1-\qt}\right)\cdot\frac{\qt}{\qo r}\\
    r(1-q)k&= (1-\quant^*)q\\
    k&= \frac{q}{r-(r-1)q}
\end{align}






\begin{proof}[Proof of \Cref{thm:upper}]
By \Cref{lem:tri}, for $\alpha \in [0.8, 0.81]$ and $r \in [2.44, 2.45]$, 
the mechanism $\mechaAR$ that posts second highest value $\vsec$ to the highest value agent with probability $\alpha$, 
and posts $r \cdot \vsec$ to the highest value agent with probability $1-\alpha$, 
the worst case distribution when the monopoly quantile is $\qo \in [0, ]$ is a triangle distribution. 



By numerical computation, for $r \in [2.44, 2.45]$, 
when $\alpha = 0.81$, the worst case distribution for mechanism $\mechaAR$
is triangle distribution with monopoly quantile at most $0.087$, 
and when $\alpha = 0.8$, the worst case distribution for mechanism $\mechaAR$
is triangle distribution with monopoly quantile at least $0.101$. 
By continuity of the program, there for $\ratio^* \approx 2.446946$, 
there exists $\alpha^*$ such that the worst case distribution 
is triangle distribution with monopoly quantile $\quant^* \approx 0.0931057$. 
By numerical computation, we have $\alpha^* \approx 0.8056405$. 
\end{proof}

==> old-files/monotone.tex <==
\begin{theorem}
Given a 2-agents, single-item revenue auction setting, with agent values drawn i.i.d. from a quadrilateral distribution (from the class described below), in order $v_{\{1\}}\geq v_{\{2\}}$.  Fix the following mechanism: with probability $\alpha\geq 2/3$, the mechanism runs the second price auction; and with probability $1-\alpha$ the mechanisms posts the price $\ratio\cdot v_{\{2\}}$ to the agent with larger value, for fixed $\ratio\geq 1$.

For a fixed quantile $\qo$, an adversary considers the class of quadrilateral distributions with peak revenue $(\qo,1)$, and any (paired) $\qt\geq \qo$ and corresponding height of the third quadrilateral point as $\qt\cdot\frac{1}{\qo r}$.

Choosing a distribution $\Qr_{\qo,\qt,\ratio}$ from this class of quadrilateral distributions, the adversary maximizes the ratio of: the revenue $\text{OPT}_{\Qr_{\qo,\qt,\ratio}}$ of the optimal mechanism which knows $\Qr_{\qo,\qt,\ratio}$; to the revenue of the algorithm when the distribution is $\Qr_{\qo,\qt,\ratio}$; by choosing $\qt$ such that the resulting quadrilateral is in fact the triangle distribution (with peak revenue $(\qo,1)$ inherited from the quadrilateral class).
\end{theorem}
\begin{proof}
The adversary is given a fixed $\qo$ by nature and $\ratio$ from the alogirthm.  Its only choice is over $\qt\geq \qo$.

From~\Cref{prop:reducetoalg} (below) using the class of quadrilateral distributions $\Qr_{\qo,\qt,\ratio}$ ranging over $\qt\geq \qo$ for $\mathcal{C}$, it is sufficient to find the quadrilateral distribution which mininizes the performance of the algorithm, and ignore the benchmark.

The rest of this proof shows that algorithm performance is increasing in $\qt$.  The consequence is that the smallest feasible choice of $\qt$ will be optimal for the adversary, which corresponds to choosing the triangle distribution as special-case quadrilateral.

For any pair of quadrilateral distributions 
$\Qr_{\qo, \qt, \ratio}$ and $\Qr_{\qo, \qt', \ratio}$ with $\qt' \geq \qt$, 
we analyze the difference in revenue for posting $\ratio\cdot v_{\{2\}}$.  Explanations for each step are given below. 
\begin{align*}
&\Rev{\mecha_{\ratio}, \Qr_{\qo, \qt', \ratio}}
- \Rev{\mecha_{\ratio}, \Qr_{\qo, \qt, \ratio}} \\
=\,& 2 \int_{\qt'}^1 \rev_{\qt'}(\ratio \cdot \valf_{\qt'}(\quant)) \, dq
- 2 \int_{\qt}^1 \revq(\ratio \cdot \valq(\quant)) \, dq \\
\geq\,& 2 \int_{\qt'}^1 \rev_{\qt'}(\ratio \cdot \valf_{\qt'}(\quant)) \, dq
- 2 \int_{\qt'}^1 \revq(\ratio \cdot \valq(\quant))\, dq 
- 2(\qt' - \qt)\\
\geq\,& 2 \int_{\qt'}^1 \rev_{\qt}(\ratio \cdot \valf_{\qt'}(\quant)) \, dq
- 2 \int_{\qt'}^1 \revq(\ratio \cdot \valq(\quant))\, dq 
- 2(\qt' - \qt)\\
\geq\,& 2 \int_{\qt'}^1 \rev_{\qt}(\ratio \cdot \valf_{\qt}(\quant)) \, dq
- 2 \int_{\qt'}^1 \revq(\ratio \cdot \valq(\quant))\, dq 
- 2(\qt' - \qt)\\
=\,& - 2(\qt' - \qt),
\end{align*}
\begin{itemize}
\item The first inequality holds because $\revq(\ratio \cdot \valq(\quant)) \leq 1$ for any $\quant$. 
\item The second inequality holds pointwise for every fixed $\quant$ and the fixed mapping $\valf_{\qt'}$ from quantile to value.  The revenue curve $\rev_{\qt'}$ weakly dominates the revenue curve $\rev_{\qt}$ from the perspective of every fixed price as input, in this case using a fixed price of $\ratio\cdot\valf_{\qt'}(\quant)$.
\item The third inequality holds pointwise for every $\quant\geq \qt'$.  Both sides of the inequality use the same revenue function $\rev_{\qt}$ (as a function of price).

We consider the respective inputs.  The left-hand side uses the price from $\ratio\cdot\valf_{\qt'}(\quant)\geq \ratio\cdot\valf_{\qt}(\quant)$ from the right-hand side.  The definition of $\qt'$ is the lower bound in quantile space such that $\ratio\cdot\valf_{\qt'}$ is at most the truncation value and posting price $\ratio\cdot\valf_{\qt'}$ trades with positive probability.  With $\quant \geq \qt$, Both $r\cdot \valf_{\qt}(\quant)$ and the smaller price $\ratio\cdot\valf_{\qt}(\quant)$ trade with positive probability when revenue (as a function of price) is instead $\rev_{\qt}$ because the two revenue curves have the same truncation value.

By the structure of quadrilateral distributions, posting a larger price results in larger revenue as long as the new price does not exceed the truncation value of the distribution.
\end{itemize}
%The second inequality holds because for any $\quant \geq \qt'$,  $\rev_{\qt'}(\ratio \cdot \valf_{\qt'}(\quant)) \geq \rev_{\qt}(\ratio \cdot \valf_{\qt'}(\quant)) \geq \rev_{\qt}(\ratio \cdot \valf_{\qt}(\quant))$. 
Therefore, we have
\begin{align*}
\frac{\partial \Rev{\mecha_{\ratio}, \Qr_{\qo, \qt, \ratio}}}{\partial \qt}
= \lim_{\qt' \to \qt} \frac{\Rev{\mecha_{\ratio}, \Qr_{\qo, \qt', \ratio}} - \Rev{\mecha_{\ratio}, \Qr_{\qo, \qt, \ratio}}}{\qt' - \qt}
\geq -2. 
\end{align*}
The revenue of the second price auction for 
quadrilateral distribution $\Qr_{\qo, \qt, \ratio}$ is 
\begin{align*}
\Rev{\mecha_1, \Qr_{\qo, \qt, \ratio}}
&= 2 \int_0^1 \rev_{\Qr_{\qo, \qt, \ratio}}(q) \, dq\\
&= 2 \int_0^{\qo} \rev_{\Qr_{\qo, \qt, \ratio}}(q) \, dq + 2 \int_{\qo}^{\qt} \rev_{\Qr_{\qo, \qt, \ratio}}(q) \, dq + 2 \int_{\qt}^1 \rev_{\Qr_{\qo, \qt, \ratio}}(q) \, dq\\
&= \qo + (\qt - \qo)(1+\frac{\qt}{\ratio\cdot \qo}) + (1-\qt)\frac{\qt}{\ratio\cdot \qo} \\
&= \qt + (1 - \qo)\frac{\qt}{\ratio\cdot \qo}. 
\end{align*}
where the third line evaluates each of the integrals as the width of the interval times the average height of the revenue curve on the interval, as each is a line segment.  Therefore, we have 
\begin{align*}
\frac{\partial \Rev{\mecha_1, \Qr_{\qo, \qt, \ratio}}}{\partial \qt}
= 1 + \frac{1 - \qo}{\ratio\cdot \qo} \geq 1.
\end{align*}
Finally, for mechanism $\mechaAR$ with $\alpha \geq \sfrac{2}{3}$, 
we have 
\begin{equation*}
\frac{\partial \Rev{\mechaAR, \Qr_{\qo, \qt, \ratio}}}{\partial \qt}
\geq \alpha - 2(1-\alpha) \geq 0. \qedhere
\end{equation*}
\end{proof}



\begin{prop}
\label{prop:reducetoalg}
Given an auction setting with $n$ agents with values drawn i.i.d. from a regular distribution and a revenue objective.  Restrict the class of distributions further to be parameterized by the peak revenue point $(\qo, R)$ on the revenue, and fix the shape of the revenue curve to the left of the peak (for all $\qt\leq \qo$).  Let $\mathcal{C}$ be any non-empty sub-set of this class.

Consider an adversarial setting in which- fixing a mechanism $\mecha$- we try to find the distribution $F$ in the restricted class $\mathcal{C}$ which maximizes the ratio of $\text{OPT}_F$ the $\mecha$ (both in expectation).  This question reduces to finding the distribution in the class which minimizes the performance of the algorithm.
\end{prop}
\begin{proof}
The optimal performance is constant over all distributions in $\mathcal{C}$, because (1) the shape of the revenue curve to the left of the peak is constant across the class, by assumption; and (2) the optimal mechanism runs the second price auction with Myerson reserve at $\qo$, and the shape of the revenue curve where it has negative virtual value has no effect on the optimal revenue.  So the question of maximizing the ratio of optimal performance to algorithm performance reduces to simply minimizing the performance of the algorithm.
\end{proof}

%\begin{fact}
%\label{fact:\qttrades}
%Given a quadrilateral distribution $\Qr_{\qo,\qt,\ratio}$.  By definition, using $\Qr_{\qo,\qt,r}$, quantiles $\qt'\geq \qt$ correspond to prices that trade with positive probability when scaled up by $\ratio$.
%\end{fact}

\newpage

For any pair of quadrilateral distributions 
$\Qr_{\qo, \qt, \ratio}$ and $\Qr_{\qo, \qt', \ratio}$ with $\qt' \geq \qt$, we analyze the difference in revenue for posting $\ratio\cdot v_{\{2\}}$, for an arbitrary number of agents $n\geq 2$.  %Explanations for each step are given below. 

The optimal auction is still a lookahead auction, and the prices are still $v_{\{2\}}$ with probability $\alpha$ and $\ratio\cdot v_{\{2\}}$ with probability $(1-\alpha)$.

We give the general form of the revenue analysis for any $n$.  As a special case for $n=2$, it reduces to the forms above.  For this extension, we use the function for revenue which integrates over conditional revenue given $q_{\{2\}}$ times the density of $q_{\{2\}}$, which is the density function $f_2(q)$ of the second-smallest (quantile) order statistic given $n$ agents.  It then must also apply the conditioning to compute revenue \textit{ex-post} of the realized $v_{\{2\}}$, as a lower bound on the largest value, which it does by dividing the integrand by $q$.

In the explanation below, let the agents be numbered in order of increasing quantile.  Given that quantiles are $U[0,1]$ draws:
    
\begin{equation}
    f_2(q) = n(n-1)\cdot q\cdot (1)\cdot (1-q)^{n-2}
\end{equation}

\noindent where $(1)$ is the density of the second-smallest quantile from the $U[0,1]$ distribution at $q$; $q$ is the probability that `agent 1' has quantile smaller than $q$; $(1-q)^{n-2}$ is the probability that each `agent $3, ..., n$' has quantile larger than $q$; and $n(n-1)$ is the combinatorial term from $n$ choices as agent 2 and then $_{n-2}\text{C}_1$ ($n-2$ choose 1) ways to choose the set of agents with smaller quantile (in this case just `agent 1').

We lower bound the revenue for posting $\ratio\cdot v_{\{2\}}$ with $n$ agents:

\begin{align*}
&\Rev{\mecha_{\ratio}, \Qr_{\qo, \qt', \ratio}}
- \Rev{\mecha_{\ratio}, \Qr_{\qo, \qt, \ratio}} \\
=\,&  \int_{\qt'}^1 \frac{\rev_{\qt'}(\ratio \cdot \valf_{\qt'}(\quant))}{q} \cdot f_2(q)\, dq
-  \int_{\qt}^1 \frac{\revq(\ratio \cdot \valq(\quant))}{q} \cdot f_2(q)\, dq \\
=\,& n(n-1)\left[ \int_{\qt'}^1 \rev_{\qt'}(\ratio \cdot \valf_{\qt'}(\quant)) \cdot \frac{q(1-q)^{n-2}}{q} \, dq
-  \int_{\qt}^1 \revq(\ratio \cdot \valq(\quant))\cdot \frac{q(1-q)^{n-2}}{q}\, dq \right]\\
\geq\,& n(n-1)\left[ \int_{\qt'}^1 \rev_{\qt'}(\ratio \cdot \valf_{\qt'}(\quant))\cdot(1-q)^{n-2}\, dq
-  \int_{\qt'}^1 \revq(\ratio \cdot \valq(\quant))\cdot (1-q)^{n-2}\frac{C_n(q)}{q}\, dq 
- (\qt' - \qt)\right]\\
\geq\,& n(n-1)\left[ \int_{\qt'}^1 \rev_{\qt}(\ratio \cdot \valf_{\qt'}(\quant))\cdot (1-q)^{n-2}\, dq
-  \int_{\qt'}^1 \revq(\ratio \cdot \valq(\quant))\cdot(1-q)^{n-2}\, dq 
- (\qt' - \qt)\right]\\
\geq\,& n(n-1)\left[ \int_{\qt'}^1 \rev_{\qt}(\ratio \cdot \valf_{\qt}(\quant))\cdot (1-q)^{n-2} \, dq
-  \int_{\qt'}^1 \revq(\ratio \cdot \valq(\quant))\cdot(1-q)^{n-2}\, dq 
- (\qt' - \qt)\right]\\
=\,& - n(n-1)\left[(\qt' - \qt)\right],
\end{align*}

\noindent where everything holds for the exact same reasons as the forms above, because the analysis above held {\em pointwise} for each $q$, and multiplying each pointwise analysis at $q$ by $C_n(q)$ which is a (positive) constant for fixed $q$ is benign to the result.  Note in particular that putting in $n=2$ gets back the exact previous analysis.

The factor of $n(n-1)$ will follow through to the analysis of the second price auction as $n(n-1)/2$, such that the result still holds for the bound: $\alpha \geq 2/3$.

==> old-files/raw-monotonicity.tex <==

\begin{lemma}\label{lem:tri}
For any $\alpha \in [\sfrac{1}{2}, 1]$ and $r \in []$, 
the mechanism $\mechaAR$ that posts second highest value $\vsec$ to the highest value agent with probability $\alpha$, 
and posts $r \cdot \vsec$ to the highest value agent with probability $1-\alpha$, 
the worst case distribution when the monopoly quantile is $\qo \in [0, ]$ is a triangle distribution. 
\end{lemma}
\begin{proof}
By \Cref{lem:quad}, without loss of generality, 
we can consider the worst case distribution as a quadrilateral distribution $\Qr_{\qo, \qt, r}$. 
% The optimal revenue for distribution $\Qr_{\qo, \qt, r}$
% is $2 - \qo$,
For simplicity, we introduce the notation $\revq(\val)$
to denote the revenue of posting price $\val$,
and $\valq(\quant)$ to denote the price $\val$ given quantile $\quant$ when the distribution is $\Qr_{\qo, \qt, r}$. 
Let $\quant^*$ be the quantile such that $r \cdot \valq(\quant^*) = \sfrac{\qt}{r\cdot \qo}$.
By construction of distribution $\Qr_{\qo, \qt, r}$, we have 
$$\quant^* = \frac{r\cdot \qt}{1+(r-1)\qt}.$$
Thus, the revenue of mechanism $\mechaAR$ given distribution $\Qr_{\qo, \qt, r}$ is as follows.  For sub-calculations substituted into this sequence, see below.
\begin{align}
\Rev{\mechaAR, \Qr_{\qo, \qt, r}}
&= 
\alpha \Rev{\mecha_1, \Qr_{\qo, \qt, r}}
+ (1-\alpha) \Rev{\mecha_r, \Qr_{\qo, \qt, r}} \\
&= 2\alpha \int_0^1 \rev_{\Qr_{\qo, \qt, r}}(q) \, dq
+ 2(1-\alpha) \int_0^1 \revq(r\cdot \valq(\quant)) \, dq \\
&= \alpha \left(\qo + (\qt - \qo)(1+\frac{\qt}{r\cdot \qo}) + (1-\qt)\frac{\qt}{r\cdot \qo}\right) \\
& \quad + 2(1-\alpha)\int_{\qt}^{\quant^*} \rev_{\Qr_{\qo, \qt, r}}(q) \, dq
+ 2(1-\alpha)\int_{\quant^*}^1 \rev_{\Qr_{\qo, \qt, r}}(q) \, dq \\
&= \alpha \left(\qo + (\qt - \qo)(1+\frac{\qt}{r\cdot \qo}) + (1-\qt)\frac{\qt}{r\cdot \qo}\right) \\
& \quad + 2(1-\alpha)\int_{\qt}^{\quant^*} \left(\frac{\qt(1-\qt)(\qo r-\qo)}{(\qt-\qo)r \qt (1-q)+q(1-\qt)(\qo r -\qt)} 
\right) \cdot \frac{\qt}{\qo}\cdot \frac{1-q}{1-\qt}\, dq \\
& \quad + 2(1-\alpha)\int_{\quant^*}^1 \frac{1}{r-(r-1)q}\cdot\frac{\qt}{\qo}\cdot\frac{1-q}{1-\qt} \, dq\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\int_{\qt}^{\quant^*} \left(\frac{1-q}{(\qt-\qo)r \qt +q(\qo r-\qt-(r-1)\qt^2)} \right)\, dq \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\int_{\quant^*}^1 \frac{1-q}{r-(r-1)q} \, dq\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-q}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln((\qt-\qo)r \qt +q(\qo r-\qt-(r-1)\qt^2) )}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right]_{\qt}^{\quant^*} \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{q}{r-1}+\frac{\ln(r-(r-1)q)}{(r-1)^2} \right]_{\quant^*}^1\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
\label{eqn:condrevqtqstar1}
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-(\quant^*-\qt)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
\label{eqn:condrevqtqstar2}
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{(\qt-\qo)r \qt +\quant^*(\qo r-\qt-(r-1)\qt^2)}{(\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right] \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\quant^*}{r-1}-\frac{\ln(r-(r-1)\quant^*)}{(r-1)^2} \right]
\end{align}

\begin{lemma}
\label{lem:condrevpos}
As a function, the quantity $h(\qt)=(\qo r-\qt-(r-1)\qt^2)$ appears in line~\eqref{eqn:condrevqtqstar1} and line~\eqref{eqn:condrevqtqstar2} in the interim revenue calculation of the quadrilateral distribution. $h(\qt)<0$ for all possible values of $\qt$.  Line~\eqref{eqn:condrevqtqstar1} is a positive term and line~\eqref{eqn:condrevqtqstar2} is a negative term (both weakly).
\end{lemma}
\begin{proof}
We give an indirect proof, ultimately by contradiction.  The range of values of $\qt$ are upperbounded by $\qt_{\max}=\qo r$.  This follows by noting that- by the description of its design- the quadrilateral distribution goes through the point $(\qt, \frac{\qt}{\qo r})$ in the revenue curve graph.  We have normalized the peak revenue of the quadrilateral distribution to be 1, so this height of the revenue curve $\qt/(\qo r)\leq 1$.

By inspection, $h(\qt_{\max})=(\qo r-\qt_{\max}-(r-1)\qt^2_{\max}) = 0-(r-1)\qt^2\leq 0$.  Further, $h(\qt)$ is continuous, and it is in the denominator of line~\eqref{eqn:condrevqtqstar1}.  If $h(\qt)$ had positive output anywhere for valid inputs of $\qt$, then by continuity, the output ``moved" from negative at the maximum input $\qt_{\max}$ through 0 to positive as $\qt$ decreases in its feasible range.  Somewhere in this critical range of $\qt$, evaluation of line~\eqref{eqn:condrevqtqstar2} would go to negative infinity.  But line~\eqref{eqn:condrevqtqstar1} and line~\eqref{eqn:condrevqtqstar2} together are the revenue component when $q_{\{2\}}$ is in the range $[\qt, \quant^*]$ and the mechanism uses $r\cdot v_{\{2\}}$ as its random price.  This quantity is positive and finite, contradicting the possibility that the evaluation of~\eqref{eqn:condrevqtqstar1} is negative infinity.

Line~\eqref{eqn:condrevqtqstar2} is negative because the $\ln$ term is negative because: $\quant^*\geq \qt$ and from the above, $h(\qt)$ is negative.
\end{proof}

\noindent We substitute out $\quant^*=r\qt / (1+(r-1)\qt)$.

\begin{align}
    1-\quant^* &= \frac{1-\qt}{1+(r-1)\qt}\\
    r-(r-1)\quant^* &= \frac{r+r(r-1)\qt}{1+(r-1)\qt}-\frac{(r-1)r\qt}{1+(r-1)\qt} =\frac{r}{1+(r-1)\qt}\\
\quant^*-\qt &= \frac{r\qt}{1+(r-1)\qt}-\frac{\qt+(r-1)\qt^2}{1+(r-1)\qt} = \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\\
&\quad \Rev{\mechaAR, \Qr_{\qo, \qt, r}}\\
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qt\cdot((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}{((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right] \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\qt}{(r-1)(1+(r-1)\qt)}-\frac{\ln\left(\frac{r}{1+(r-1)\qt} \right)}{(r-1)^2} \right]\\
\intertext{(we replace the third line using \Cref{cal:simpmonst} below)}
&= \alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right) \\
& \quad + 2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.\\
&\quad \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right] \\
& \quad + 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\qt}{(r-1)(1+(r-1)\qt)}-\frac{\ln\left(\frac{r}{1+(r-1)\qt} \right)}{(r-1)^2} \right]
\end{align}

\begin{calc}
\label{cal:simpmonst}
\begin{align*}
& \quad  \frac{r \qt\cdot((\qt-\qo)(1+(r-1)\qt) +(\qo r-\qt-(r-1)\qt^2))}{((\qt-\qo)r \qt +\qt(\qo r-\qt-(r-1)\qt^2))\cdot(1+(r-1)\qt)}   \\
= &\quad \frac{r \qt\cdot((-\qo)(1+(r-1)\qt) +\qo r)}{(r\qt^2-\qt^2-(r-1)\qt^3)\cdot(1+(r-1)\qt)} \\
= &\quad \frac{r \qt\cdot(\qo(r-1)(1-\qt))}{(\qt^2(r-1)(1-\qt))\cdot(1+(r-1)\qt)} =  \frac{r \qo}{\qt\cdot(1+(r-1)\qt)}  \quad \bullet
\end{align*}
\end{calc}

\noindent We handle each derivative of the additive terms before combining.  The end of the calculation for each additive term is market with $\bullet$.

\begin{align}
    & \quad \partial \left(\alpha \left(\qt + (1 - \qo)\frac{\qt}{r\cdot \qo} \right)  \right) / \partial \qt =  \alpha\left(1 + \frac{1-\qo}{r\qo}\right)=\alpha\left(\frac{1+(r-1)\qo } { r\qo} \right)\quad \bullet\\
    %1-\quant^* &= \frac{1-\qt}{1+(r-1)\qt}\\
    %r-(r-1)\quant^* &= \frac{r(1+(r-1)\qt)}{1+(r-1)\qt}-\frac{(r-1)(1-\qt)}{1+(r-1)\qt} =\frac{r+r(r-1)\qt -r+r\qt +1-\qt}{1+(r-1)\qt}=\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt}\\
    & \quad \partial \left( 2(1-\alpha)\frac{\qt}{\qo(1-\qt)}\cdot \left[
\frac{1-\qt}{(r-1)(1+(r-1)\qt)}-\frac{\ln\left(\frac{r}{1+(r-1)\qt} \right)}{(r-1)^2} \right]\right) /\partial \qt\\
\intertext{(multiply the $\qt/(\qo(1-\qt)$ term into the brackets)}
    = & \quad \partial \left( 2(1-\alpha)\cdot \left[
\frac{\qt}{\qo(r-1)(1+(r-1)\qt)}-\frac{\qt\ln\left(\frac{r}{1+(r-1)\qt} \right)}{\qo(1-\qt)(r-1)^2} \right]\right) /\partial \qt\\
\intertext{(evaluate the partial derivative)}
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)\qt}{\qo(r-1)^2(1-\qt)}\cdot\left[0-\frac{r-1}{1+(r-1)\qt} \right]\\
    &\quad -\frac{2(1-\alpha)}{\qo(r-1)^2}\cdot\ln\left(\frac{r}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
\intertext{(add and subtract 1 inside the $\ln$)}
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}+\frac{2(1-\alpha)\qt}{\qo(r-1)(1-\qt)}\cdot\left[\frac{1}{1+(r-1)\qt} \right]\\
    &\quad -\frac{2(1-\alpha)}{\qo(r-1)^2}\cdot\ln\left(1+\frac{r-1-(r-1)\qt}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
\intertext{(use the bound $-\ln(1+x)\geq -x$ for all $x>-1$, and in particular for $[r/ (1+(r-1)\qt)-1]\geq 0$ because the denominator is a convex combination of 1 and $r\geq 1$)}
    \geq & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}+\frac{2(1-\alpha)\qt}{\qo(r-1)(1-\qt)}\cdot\left[\frac{1}{1+(r-1)\qt} \right]\\
    &\quad -\frac{2(1-\alpha)}{\qo(r-1)^2}\cdot\left(\frac{(r-1)(1-\qt)}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
\intertext{(cancel $(r-1)(1-\qt)$) in the third term}
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}+\frac{2(1-\alpha)\qt}{\qo(r-1)(1-\qt)}\cdot\left[\frac{1}{1+(r-1)\qt} \right]\\
    &\quad -\frac{2(1-\alpha)}{\qo(r-1)}\cdot\left(\frac{1}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)}\\
\intertext{(combine the last two additive terms and then cancel $(1-\qt)$)}
    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)}{\qo(r-1)}\cdot\left[\frac{1}{1+(r-1)\qt} \right]\\
\intertext{(multiply second term top-and-bottom by $(1+(r-1)\qt)$ and do final simplification)}
    = & \quad -\left(\frac{2(1-\alpha)}{\qo(r-1)}\right)\cdot\frac{(r-1)\qt}{(1+(r-1)\qt)^2}= -\left(\frac{2(1-\alpha)}{\qo}\right)\cdot\frac{\qt}{(1+(r-1)\qt)^2}\quad \bullet
%    = & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)^2}\right)\cdot\frac{r-1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)}{q(r-1)^2}\cdot\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)\cdot\frac{1}{(1-\qt)^2}\\
%    &\quad -\frac{2(1-\alpha)\qt}{q(r-1)^2(1-\qt)}\cdot\left[\frac{r(r-1)}{(r^2\qt+(1-\qt))(1+(r-1)\qt)}\right]\\
%    \geq & \quad \left(\frac{2(1-\alpha)}{\qo(r-1)^2}\right)\cdot\frac{r-1}{(1+(r-1)\qt)^2}-\frac{2(1-\alpha)}{q(r-1)^2}\cdot\frac{1}{(1-\qt)^2}\\
%    &\quad -\frac{2(1-\alpha)\qt}{q(r-1)^2(1-\qt)}\cdot\left[\frac{r(r-1)}{(r^2\qt+(1-\qt))(1+(r-1)\qt)}\right]\\
%\intertext{by $\ln\left(\frac{r^2\qt+(1-\qt)}{1+(r-1)\qt} \right)\leq \ln\left(\frac{r^2\qt+r(1-\qt)}{1+(r-1)\qt} \right)= \ln r \leq 1$, assuming $1\leq r \leq \exp(1)$; however, perhaps another substitution using the Taylor Series approximation bounds on $\ln$-function is more appropriate}
    %= & \frac{2(1-\alpha)}{\qo}\cdot\frac{(r-1)(1-\qt)^2(r^2\qt+(1-\qt))-(r^2\qt+(1-\qt))(1+(r-1)\qt)^2 }{(r-1)^2(1-\qt)^2(r^2\qt+(1-\qt)(1+(r-1)\qt)^2}\\
    %& \quad + \frac{2(1-\alpha)}{\qo}\cdot\frac{-(r-1)(1-\qt)(1+(r-1)\qt)r}{(r-1)^2(1-\qt)^2(r^2\qt+(1-\qt)(1+(r-1)\qt)^2}
\end{align}

\begin{align}
    & \quad \partial \left(2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.
    \right.\\
    &\quad \left. \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right]\right)/\partial \qt\\
\intertext{(take the partial derivative which- with various applications of product rule and chain rule- requires the next 7 lines)}
    =& \quad \left(2(1-\alpha)\frac{2\qt(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right.\right.
    \right.\\
    &\quad \left. \left.\left.+\frac{\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2} \right]\right]\right)\\
    &\quad +\left(2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{+\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot (-1-2(r-1)\qt)\right.\right.
    \right.\\
    &\quad +\frac{+\left( \frac{(r-1)\qt(1-\qt)}{(1+(r-1)\qt)^2}\cdot(r-1)\right)}{(\qo r-\qt-(r-1)\qt^2)}+\frac{-\left( \frac{(r-1)(1-2\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\\
    &\quad +\frac{\left(-1\cdot((\qo r-\qt)+(1-\qt))\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^2}\\
    &\quad +\frac{-2\cdot\left((\qo r-\qt)(1-\qt)\right)\cdot \ln\left(\frac{r \qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^3}\cdot(-1-2(r-1)\qt )\\
    &\quad \left.\left.\left.-\frac{\left((\qo r-\qt)(1-\qt)\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot\left(\frac{1+2(r-1)\qt} {\qt(1+(r-1)\qt)}\right)\right]\right]\right)
\intertext{(we consolidate all lines with $\ln$ terms using \Cref{cal:consln}, which includes using the respective $2\qt$ and $\qt^2$ factors outside the brackets)}
    \geq& \quad \left(2(1-\alpha)\frac{2\qt(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{-\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\right]\right]\right)\\
    &\quad +\left(2(1-\alpha)\frac{\qt^2(\qo r-\qo)}{\qo}\cdot \left[\left[ \frac{+\left( \frac{(r-1)\qt(1-\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot (-1-2(r-1)\qt)\right.\right.
    \right.\\
    &\quad +\frac{+\left( \frac{(r-1)\qt(1-\qt)}{(1+(r-1)\qt)^2}\cdot(r-1)\right)}{(\qo r-\qt-(r-1)\qt^2)}+\frac{-\left( \frac{(r-1)(1-2\qt)}{1+(r-1)\qt}\right)}{(\qo r-\qt-(r-1)\qt^2)}\\
    &\quad \left.\left.\left.-\frac{\left((\qo r-\qt)(1-\qt)\right)}{(\qo r-\qt-(r-1)\qt^2)^2}\cdot\left(\frac{1+2(r-1)\qt} {\qt(1+(r-1)\qt)}\right)\right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{\ln\left(\frac{r\qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(expand the first four lines to re-organize with common denominator, in order, again absorbing the $2\qt$ and $\qt^2$ factors outside the brackets; note that the term with factor $(1-2\qt)$ is split into two terms using $((1-\qt)-\qt)$ to simplify the next step)}%; add and subtract 1 within the $\ln$ term at the end)}
    = &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{1}{(\qo r-\qt -(r-1)\qt^2)^2(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -2\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.
    \\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)^2(1-\qt)+ \qt^3(r-1)(1+(r-1)\qt)\\
    &\quad - \qt^2(r-1)(1-\qt)(1+(r-1)\qt)\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{\ln\left(\frac{r\qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(combine some terms)}
    = &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{1}{(\qo r-\qt -(r-1)\qt^2)^2(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -3\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.
    \\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)r\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{\ln\left(\frac{r\qo}{\qt\cdot(1+(r-1)\qt)} \right)}{(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(we now work towards relaxing the $\ln$ term by add-and-subtract 1 inside of it, and multiplying top-and-bottom by $(-1)$; this makes the denominator positive (as by \Cref{lem:condrevpos} the quantity $(\qo r-\qt-(r-1)\qt^2)^3$ is negative); which sets us up to lower bound a $-\ln(\cdot)$ term)}
    = &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{1}{(\qo r-\qt -(r-1)\qt^2)^2(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -3\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.
    \\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)r\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{-\ln\left(1+\frac{r\qo-\qt\cdot(1+(r-1)\qt)}{\qt\cdot(1+(r-1)\qt)} \right)}{-(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(we use the relaxation $-\ln(1+x)\geq -x$, which we can do if the rest of the factors combine to be positive, which they do: the denominator term $-(\qo r-\qt-(r-1)\qt^2)$ is positive by \Cref{lem:condrevpos} and the triple-brackets term is argued to be positive where it is derived in \Cref{cal:consln}; conveniently, the term composed of the last three lines started positive and will remain positive below)}
    \geq &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{1}{(\qo r-\qt -(r-1)\qt^2)^2(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -3\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.
    \\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)r\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{-\left(\frac{r\qo-\qt\cdot(1+(r-1)\qt)}{\qt\cdot(1+(r-1)\qt)}\right)}{-(\qo r-\qt-(r-1)\qt^2)^3 } \right)\cdot\\
    &\quad [[[\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)]]]
\intertext{(in preparation to combine, multiply the first term (the first five lines) top-and-bottom by $-1(\qo r-\qt-(r-1)\qt^2)$; multiply the second term (last three lines) top-and-bottom by $(1+(r-1)\qt)^2$ and cancel a factor top-and-bottom of $\qt$)}
    \geq &\quad \left (2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot\left(\frac{-(\qo r-\qt-(r-1)\qt^2)}{(-(\qo r-\qt -(r-1)\qt^2)^3)(1+(r-1)\qt)^2} \right)\cdot\right.\\ 
    &\quad \left[ \left[ -3\qt^2(r-1)(1-\qt)(1+(r-1)\qt)\right.\right.\\
    &\quad - \qt^3(r-1)(1-\qt)(1+(r-1)\qt)(1+2(r-1)\qt)\\
    &\quad + \qt^3(r-1)r\\
    &\quad \left.\left.\left.- \qt(\qo r -\qt)(1-\qt) (1+(r-1)\qt)(1+2(r-1)\qt) \right]\right]\right)\\
    &\quad +2(1-\alpha)\frac{(\qo r-\qt)}{\qo}\cdot \left(\frac{(\qt\cdot(1+(r-1)\qt)- r \qo)(1+(r-1)\qt)}{(-(\qo r-\qt-(r-1)\qt^2)^3)(1+(r-1)\qt)^2 } \right)\cdot\\
    &\quad [[[(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^3(\qo r-\qt)(r-1)+\qt^3(1-\qt)(r-1)]]]
\end{align}

\end{proof}

\begin{calc}
\label{cal:consln}
\begin{align*}
    &\quad +2\qt(\qo r-\qt)(1-\qt)((\qo r-\qt)-(r-1)\qt^2)\\
    &\quad + 2\qt^2(\qo r-\qt)(1-\qt)(1+2(r-1)\qt)\\
    &\quad - \qt^2((\qo r-\qt)+(1-\qt))((\qo r-\qt)-(r-1)\qt^2)\\
    = & \quad 2\qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+(r-1)\qt^2\right]\\
    &\quad - \qt^2(\qo r-\qt)((\qo r-\qt)-(r-1)\qt^2)-\qt^2(1-\qt)((\qo r-\qt)-(r-1)\qt^2)\geq0\\
\intertext{{\em (where the inequality follows because the positive term (first row) has all positive factors, and each ``negative" term (second row) has a factor of $(\qo r-\qt)-(r-1)\qt^2)<0$ by \Cref{lem:condrevpos}, such that they are actually positive; we continue manipulation to further simplify substitution into the main calculation of the derivative)}}
    \Leftrightarrow & \quad \qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-\qt)\\
    &\quad - \qt^2(\qo r-\qt)((\qo r-\qt)-(r-1)\qt^2)+\qt^4(1-\qt)(r-1)\geq 0\\
    \Leftrightarrow & \quad \qt(\qo r-\qt)(1-\qt)\left[(\qo r-qt)+\qt+2(r-1)\qt^2\right]+\qt(\qo r-\qt)^2(1-2\qt)\\
    &\quad + \qt^4(\qo r-\qt)(r-1)+\qt^4(1-\qt)(r-1)\geq 0 \quad \bullet
\intertext{{\em (where each further manipulation has been re-arrangement of the left-hand side with equality such that it is necessarily still non-negative overall; however, the third term individually is possibly negative due to the $(1-2\qt)$ term)}}
\end{align*}
\end{calc}



\noindent\textbf{The following gives sub-calculations in support of the preceding.}

\noindent We give the identity for $\quant^*$.  We can calculate the height of the quadrilateral revenue curve at $\quant^*\in[\qt,1]$ from two formulas each using $\quant^*$.  We can set them equal and solve.
\begin{align}
    \text{height at}~\quant^*\in[\qt,1]:\quad \quant^*\cdot\frac{1}{\qo r^2} &= \frac{\qt}{\qo r}\cdot\frac{1-\quant^*}{1-\qt}\\
    \quant^*(1-\qt) &= r \qt(1-\quant^*)\\
    \quant^*(1-\qt) &= r\qt-r\qt \quant^*\\
    \quant^*\left((1-\qt)+r \qt \right) &= r\qt\\
    \quant^* &= \frac{\qt r}{(1-\qt)+\qt r} = \frac{\qt r}{1+(r-1)\qt}
\intertext{we note this also induces for substitution:}
    1-\quant^* &= \frac{1-\qt}{1+(r-1)\qt}\\
    r - (r-1)\quant^* &= \frac{r(1+(r-1)\qt)}{1+(r-1)\qt}-\frac{(r-1)(1-\qt)}{1+(r-1)\qt}\\
    &= \frac{r + r(r-1)\qt-r+r\qt+1-\qt}{1+(r-1)\qt} = \frac{r^2\qt +(1-\qt)}{1+(r-1)\qt}
\end{align}

\noindent Given the quadrilateral curve, the value $v^*$ associated with quantile $q\in[\quant^*,1]$, and the value $v'$ for $q\in[\qt,\quant^*]$, are
\begin{align}
    v^*(q) &= \frac{1}{q}\cdot\left(\frac{1-q}{1-\qt}\right)\cdot\frac{\qt}{\qo r}\\
    v'(q) &= \left(\frac{\qt-\quant^*}{\qt-\qo}\right)\left(1-\frac{\qt}{\qo r}\right)+\frac{\qt}{\qo r}
\intertext{A price scaled up by a factor of $r$ given $q\in[\qt,1]$ is}
    r\cdot v^*(q) &= \frac{\qt}{\qo q}\cdot\left(\frac{1-q}{1-\qt}\right)
\end{align}

\noindent The following {\em does not} condition the ``probability of sale" to try to sell to an agent with quantile smaller than the input $q$; this quantity follows from the ending calculated terms, divided by $q$.  The probability of sale $k$ given $q\in[\qt,\quant^*]$ and corresponding value as price scaled up by $r$ can be found from the intersection of
\begin{align}
    \frac{\qt}{\qo q}\left(\frac{1-q}{1-\qt}\right)k & = \left(\frac{\qt-\quant^*}{\qt-\qo}\right)\left(1-\frac{\qt}{\qo r}\right) + \frac{\qt}{\qo r}\\
    (\qt-\qo)\frac{r\qt}{q}(1-q)k &= (\qt-\quant^*)(1-\qt)(\qo r-\qt)+\qt(\qt-\qo)(1-\qt)\\
    \left[(\qt-\qo)\frac{r\qt}{q}(1-q)+(1-\qt)(\qo r-\qt) \right]k &= \qt(1-\qt)(\qo r - \qo)\\
    k&= \frac{q\qt(1-\qt)(\qo r-\qo)}{(\qt-\qo)r\qt(1-q)+q(1-\qt)(\qo r-\qt)}
\end{align}

\noindent Finally with similar technique, we determine the probability of sale for the scale-up price given $q\in[\quant^*,1]$:

\begin{align}
    \frac{\qt}{\qo q}\left(\frac{1-q}{1-\qt}\right)k &= \left(\frac{1-\quant^*}{1-\qt}\right)\cdot\frac{\qt}{\qo r}\\
    r(1-q)k&= (1-\quant^*)q\\
    k&= \frac{q}{r-(r-1)q}
\end{align}



==> old-files/setting.tex <==


\section{Setting}
\label{s:setting}

%%
%% summary of problem and paper.
%%

In this paper, we consider the seller tries to sell a single item to two buyers. 
We first start with prior independent mechanism design, where
the value of the buyers $\vali$ for $i \in \{1, 2\}$ 
are drawn from independent and identical distribution $\dist$. 
The seller does not know the distribution $\dist$, 
but the seller knows the set of possible distributions $\cF$
and the seller wants to approximate the optimal revenue for all possible distributions $\dist \in \cF$. 
By slightly abusing the notation, 
we also use $\dist(\val)$ to denote the cumulative distribution. 
Let $\quantf_{\dist}(\val) = 1 - \dist(\val)$ be the quantile of the agent. 
% Let $\density(\val)$ be the density function given distribution $\dist$. 
The set of mechanisms we focus on in this paper are revelation mechanisms. 
For any dominant strategy incentive compatible revelation mechanism $\mech$, 
we use $\Rev{\mech, \dist}$ to denote the revenue of the mechanism 
when the prior distribution is $\dist$, 
and we use $\OPT(\dist)$ to denote the optimal revenue when the distribution is $\dist$. 
The objective of the seller is to find the mechanism that minimize the maximum ratio between the optimal revenue and the revenue of the mechanism, 
i.e., find mechanism $\mech$ that solves
$$\min_{\mecha}\max_{\dist \in \cF} \frac{\OPT(\dist)}{\Rev{\mech, \dist}}$$

For each agent with distribution $\dist$, 
we use $\valf_{\dist}(\quant)$ to denote the value of the agent that corresponds to quantile $\quant$.
The revenue curve for this agent is a mapping from the probability the item is sold to this agent, 
to the revenue obtained from posting a price to this agent. 
That is, we define the revenue curve 
$\rev_{\dist}(\quant) = \quant \cdot \valf_{\dist}(\quant)$. 

The set of distributions $\cF$ we focus on in this paper is the set of regular distributions, 
i.e., the set of distributions whose revenue curve $\rev$ is concave. 
There are two families of regular distributions that are crucial for our analysis. 
The family of triangle distributions is characterized by two parameters, 
$\bar{\val}$ and $\qo$. 
We use $\Tr_{\bar{\val}, \qo}$ to denote the specific triangle distribution with those two parameters. 
The quantile function for the triangle distribution $\Tr_{\bar{\val}, \qo}$ is
\begin{equation*}
\quantf_{\Tr_{\bar{\val}, \qo}}(\val) = 
\begin{cases}
\frac{\bar{\val}\qo}{\bar{\val}\qo + \val(1-\qo)} & \val \leq \bar{\val}\\
0 & \val > \bar{\val}
\end{cases}
\end{equation*}
Another family of distribution is called the quadrilateral distributions, 
which is characterized by $\qo, \qt, \bar{\val}$ and $r$. 
We use $\Qr_{\bar{\val}, \qo, \qt, r}$ to denote the specific quadrilateral distribution with those four parameters. 
The constraints on the parameters is that 
$r \geq 1$
and 
$\frac{\qo r}{\qo r + (1-\qo)}
\leq \qt \leq r \qo$. 
The quantile function for the quadrilateral distribution $\Qr_{\bar{\val}, \qo, \qt, r}$ is
\begin{equation*}
\quantf_{\Qr_{\bar{\val}, \qo, \qt, r}}(\val) = 
\begin{cases}
\frac{\bar{\val}\qt}{\bar{\val}\qo + \val r(1-\qt)} & \val < \sfrac{\bar{\val}}{r}\\
\frac{\sfrac{\bar{\val} \qt}{r} 
- \sfrac{\qt(\bar{\val} \qo - \sfrac{\bar{\val} \qt}{r})}
{(\qo - \qt)}}
{v - \sfrac{(\bar{\val} \qo - \sfrac{\bar{\val} \qt}{r})}
{(\qo - \qt)}} 
& \sfrac{\bar{\val}}{r} \leq \val \leq \bar{\val}\\
0 & \val > \bar{\val}
\end{cases}
\end{equation*}

\begin{figure}[t]
\centering
\input{fig/quad.tex}
\caption{\label{f:quad}
The revenue curve for quadrilateral distribution $\Qr_{\qo, \qt, r}$. }
\end{figure}
For simplicity, if $\bar{\val}$ is normalized such that $\bar{\val} \qo = 1$, 
we use $\Tr_{\qo}$ to denote the corresponding triangle distribution, 
and $\Qr_{\qo, \qt, r}$ to denote the corresponding quadrilateral distribution. 
We also use $\tri$ to denote the set of triangle distributions, 
and $\reg$ to denote the set of regular distributions. 
The revenue curve for quadrilateral distribution $\Qr_{\qo, \qt, r}$. 
is depicted in \Cref{f:quad}. 
% For notation convenience, 
% let $\regular$ be the set of regular distributions, 
% $\tri$ be the set of triangle distributions,
% and $\la$ be the set of deterministic look ahead mechanisms. 

Given any revelation mechanism $\mecha$, 
let $\alloci(\vali, \vali[-i])$ be the allocation for agent $i$
given the values are $\vali$ and $\vali[-i]$. 
A family of mechanisms that are of general interests in our setting are the family of scale invariant mechanisms.
A mechanism is scale invariant if for each agent $i$
and any constant $\alpha > 0$, 
$\alloci(\alpha\vali, \alpha\vali[-i]) = \alloci(\vali, \vali[-i])$. 
In \citet{AB-18}, the authors prove that the optimal scale invariant mechanism is the optimal prior independent mechanism among a family of 
simple\footnote{They show that if $\lim_{\alpha\to 0} \alloci(\alpha\vali, \alpha\vali[-i])$ always exists, 
then the optimal scale invariant mechanism is the optimal prior independent mechanism.} mechanisms.
In our paper, we will also focus on the family of scale invariant mechanisms, 
and find the optimal mechanism in this family. 
For notation convenience, we use $\scalei$ to denote the family of scale invariant mechanisms
We conjecture that the assumption on scale invariant is not necessary for the optimality. 

% Let $\scalei$ be the set of scale free mechanisms and $\sfl$ be the set of scale free and look ahead mechanisms. 

% We use $\valf_{\dist}(\quant)$ to denote the value corresponds to quantile $\quant$
% given distribution $\dist$,
% and use $\rev_{\dist}(\quant) = \val_{\dist}(\quant) \cdot \quant$ to denote the optimal revenue of distribution $\dist$ 
% given quantile constraint $\quant$. 



Another model closely related to prior independent mechanism design is the prior free mechanism design. 
In this setting, there is no prior distribution on the valuation profile of the agents. 
The objective is to optimize the performance of the mechanism on every valuation profile. 
An important question in the regime is to design reasonable benchmark. 
First, we want the benchmark to be normalized. 
Suppose the family of mechanism we consider is $\bM$
and the objective function is $\obj(\mecha, \vals)$
given any mechanism $\mecha \in \bM$ and valuation profile $\vals$. 
We say that the benchmark $\benchmark$ is normalized 
with respect a family of distribution $\cF$ if 
$\expect[\vals \sim \dist]{\benchmark(\vals)} \geq \OPT(\dist)$ for any $\dist \in \cF$.
Here when we write $\vals \sim \dist$, 
we mean that the value of each agent in valuation profile $\vals$ 
is drawn independently identically from distribution $\dist$. 
Another criterion for the benchmark is that we want the resolution of the optimal mechanism
comparing to the benchmark to be small, 
which means there exists a mechanism that has small approximation ratio comparing to the benchmark, 
i.e., we want a benchmark that solves 
\begin{equation*}
\min_{\benchmark\in \cB} \min_{\mecha \in \bM} \max_{\vals} 
\frac{\benchmark(\vals)}{\obj(\mecha, \vals)},
\end{equation*}
where $\cB$ is the set of normalized benchmarks. 
In literature, a simply heuristic for finding the optimal benchmark is to 
find the normalized benchmark that minimize the gap
between the expected benchmark and the optimal objective, i.e., 
find a benchmark that solves  
\begin{align*}
\min_{\benchmark\in \cB} \max_{\dist \in \cF} 
\frac{\expect[\vals\sim \dist]{\benchmark(\vals)}}{\OPT(\dist)}.
\end{align*}

% Let the family of distribution be $\cF$, 
% and the objective function be $\obj(\cdot)$. 
% Let $\cB = \{\benchmark : \expect[\val\sim \dist]{\benchmark(\val)} \geq \OPT(\dist), \forall \dist \in \cF\}$
% be the set of normalize benchmark. 
% For optimizing prior free performance, we have 
% \begin{equation*}
% \gamma = 
% \min_{\benchmark\in \cB} \min_{\mecha \in \bM} \max_{\val} 
% \frac{\benchmark(\val)}{\obj(\mecha, \val)}
% \end{equation*}

% For optimal prior independent mechanism, we have
% \begin{equation*}
% \beta = 
% \min_{\mecha \in \bM} \max_{\dist \in \cF} 
% \frac{\OPT(\dist)}{\expect[\val\sim \dist]{\obj(\mecha, \val)}}
% \end{equation*}




==> prelim.tex <==
\section{Preliminaries}
\label{s:prelim}

In this paper, we mainly focus on prior-free benchmark optimization. 
In this setting, 
% we want to compare the performance of the mechanism and the benchmark pointwise for each valuation profile. 
% there is no prior distribution on the valuation profile of the agents. 
the objective is to approximate the benchmark for the payoff of the mechanism designer 
on every realization of the valuation profile. 
An important question in the regime is to design the reasonable benchmark. 
First, we want the benchmark to be normalized. 
For any mechanism $\mecha$, 
% and any valuation profile~$\vals$, 
the payoff of the mechanism designer 
under the input of any valuation profile~$\vals$
is denoted as $\mecha(\vals)$.
% $\mecha(\vals)$. 
For any distribution $\dist$ over the valuation profile, 
let $\mecha(\dist) = \expect[\vals \sim \dist]{\mecha(\vals)}$ 
be the expected payoff of the mechanism designer given mechanism $\mecha$ and distribution $\dist$. 
Let $\OPT_{\dist}$ be the optimal mechanism that maximize payoff of the mechanism designer 
obtained by any feasible mechanism with access to the underlying distribution $\dist$, 
and denote $\OPT_{\dist}(\dist)$
as the corresponding expected payoff. 
Then, we say that a benchmark $\benchmark$ is normalized 
with respect a family of distributions $\feasibleDist$ 
if 
$\expect[\vals \sim \dist]{\benchmark(\vals)} \geq \OPT_{\dist}(\dist)$ 
for all distributions $\dist \in \feasibleDist$.
We use $\normBenchmark(\feasibleDist)$ to denote the set of normalized benchmark with respect a family of distributions $\feasibleDist$. 

% let $\OPT_{\dist}(\dist)$ be the optimal expected objective obtained by any feasible mechanism with access to the underlying distribution $\dist$. 
% In this paper, the set of feasible mechanism we focus on is the set of incentive compatible and 
% individual rational mechanisms. 
% Individual rational means for each agent $i$, 
% her expected utility $\expect[\val_{-i}]{\utili(\mech(\vali, \vali[-i]); \vali)}$ 
% given the outcome of the mechanism $\mech(\vali, \vali[-i])$ and her valuation $\vali$ is always non-negative, 
% and incentive compatible means truthfully reporting her valuation is the utility maximization strategy, that is, 
% for each agent $i$, 
% we have
% $\expect[\val_{-i}]{\utili(\mech(\vali, \vali[-i]); \vali)}
% \geq \expect[\val_{-i}]{\utili(\mech(\vali', \vali[-i]); \vali)}$.


% Suppose the family of mechanism we consider is $\feasibleMecha$
% Here when we write $\vals \sim \dist$, 
% we mean that the value of each agent in valuation profile $\vals$ 
% is drawn independently identically from distribution $\dist$. 
Another criterion for the designing better benchmark is that we want the resolution of the optimal mechanism
comparing to the benchmark to be small, 
which means there exists a prior-free mechanism that has small approximation ratio comparing to the benchmark, 
i.e., letting $\feasibleMecha$ be the set of feasible prior-free mechanisms, 
we want a benchmark that solves 
\begin{equation*}
\min_{\benchmark\in \normBenchmark(\feasibleDist)} \min_{\mecha \in \feasibleMecha} \max_{\vals} 
\frac{\benchmark(\vals)}{\mecha(\vals)}
\end{equation*}
for a fixed family of distributions $\feasibleDist$.
We refer to this ratio of the above program as the resolution of the optimal benchmark.
In the program, we implicitly make the constraint that the valuation profile should come from the support of some distribution $\dist \in \feasibleDist$. 
This is a hard problem to solve.
A heuristic for finding the optimal benchmark is to 
find the normalized benchmark that minimize the gap
between the expected payoff from the benchmark and the optimal payoff, i.e., 
find a benchmark that solves  
\begin{align*}
\min_{\benchmark\in \normBenchmark(\feasibleDist)} \max_{\dist \in \feasibleDist} 
\frac{\expect[\vals\sim \dist]{\benchmark(\vals)}}{\OPT_{\dist}(\dist)}.
\end{align*}

As we will show in the following section, optimal prior-free benchmark 
is equivalent to solving the prior-independent mechanism design problem. 
In this setting, the mechanism designer knows the set of possible distributions $\feasibleDist$, 
but she does not know the true distribution $\dist \in \feasibleDist$. 
The goal is to approximate the optimal objective for all distributions in $\feasibleDist$,
i.e., the mechanism designer wants to find the mechanism that solves
$$\min_{\mecha \in \feasibleMecha}\max_{\dist \in \feasibleDist} \frac{\OPT_{\dist}(\dist)}{\mecha(\dist)},$$
where $\feasibleMecha$ is the set of feasible prior-independent mechanism considered by the designer. 
% and $\mecha(\dist) = \expect[\vals \sim \dist]{\mecha(\vals)}$
% is the expected objective for mechanism $\mech$ under distribution~$\dist$. 






%%
%% summary of problem and paper.
%%





% In this paper, we consider the seller tries to sell a single item to two buyers. 
% We first start with prior-independent mechanism design, where
% the value of the buyers $\vali$ for $i \in \{1, 2\}$ 
% are drawn from independent and identical distribution $\dist$. 
% The seller does not know the distribution $\dist$, 
% but the seller knows the set of possible distributions $\feasibleDist$
% and the seller wants to approximate the optimal revenue for all possible distributions $\dist \in \feasibleDist$. 
% By slightly abusing the notation, 
% we also use $\dist(\val)$ to denote the cumulative distribution. 
% Let $\quantf_{\dist}(\val) = 1 - \dist(\val)$ be the quantile of the agent. 
% % Let $\density(\val)$ be the density function given distribution $\dist$. 
% The set of mechanisms we focus on in this paper are revelation mechanisms. 
% For any dominant strategy incentive compatible revelation mechanism $\mech$, 
% we use $\Rev{\mech, \dist}$ to denote the revenue of the mechanism 
% when the prior distribution is $\dist$, 
% and we use $\OPT_{\dist}(\dist)$ to denote the optimal revenue when the distribution is $\dist$. 
% The objective of the seller is to find the mechanism that minimize the maximum ratio between the optimal revenue and the revenue of the mechanism, 
% i.e., find mechanism $\mech$ that solves
% $$\min_{\mecha}\max_{\dist \in \feasibleDist} \frac{\OPT_{\dist}(\dist)}{\Rev{\mech, \dist}}$$

% For each agent with distribution $\dist$, 
% we use $\valf_{\dist}(\quant)$ to denote the value of the agent that corresponds to quantile $\quant$.
% The revenue curve for this agent is a mapping from the probability the item is sold to this agent, 
% to the revenue obtained from posting a price to this agent. 
% That is, we define the revenue curve 
% $\rev_{\dist}(\quant) = \quant \cdot \valf_{\dist}(\quant)$. 

% The set of distributions $\feasibleDist$ we focus on in this paper is the set of regular distributions, 
% i.e., the set of distributions whose revenue curve $\rev$ is concave. 
% There are two families of regular distributions that are crucial for our analysis. 
% The family of triangle distributions is characterized by two parameters, 
% $\bar{\val}$ and $\qo$. 
% We use $\Tr_{\bar{\val}, \qo}$ to denote the specific triangle distribution with those two parameters. 
% The quantile function for the triangle distribution $\Tr_{\bar{\val}, \qo}$ is
% \begin{equation*}
% \quantf_{\Tr_{\bar{\val}, \qo}}(\val) = 
% \begin{cases}
% \frac{\bar{\val}\qo}{\bar{\val}\qo + \val(1-\qo)} & \val \leq \bar{\val}\\
% 0 & \val > \bar{\val}
% \end{cases}
% \end{equation*}
% Another family of distribution is called the quadrilateral distributions, 
% which is characterized by $\qo, \qt, \bar{\val}$ and $r$. 
% We use $\Qr_{\bar{\val}, \qo, \qt, r}$ to denote the specific quadrilateral distribution with those four parameters. 
% The constraints on the parameters is that 
% $r \geq 1$
% and 
% $\frac{\qo r}{\qo r + (1-\qo)}
% \leq \qt \leq r \qo$. 
% The quantile function for the quadrilateral distribution $\Qr_{\bar{\val}, \qo, \qt, r}$ is
% \begin{equation*}
% \quantf_{\Qr_{\bar{\val}, \qo, \qt, r}}(\val) = 
% \begin{cases}
% \frac{\bar{\val}\qt}{\bar{\val}\qo + \val r(1-\qt)} & \val < \sfrac{\bar{\val}}{r}\\
% \frac{\sfrac{\bar{\val} \qt}{r} 
% - \sfrac{\qt(\bar{\val} \qo - \sfrac{\bar{\val} \qt}{r})}
% {(\qo - \qt)}}
% {v - \sfrac{(\bar{\val} \qo - \sfrac{\bar{\val} \qt}{r})}
% {(\qo - \qt)}} 
% & \sfrac{\bar{\val}}{r} \leq \val \leq \bar{\val}\\
% 0 & \val > \bar{\val}
% \end{cases}
% \end{equation*}

% \begin{figure}[t]
% \centering
% \input{fig/quad.tex}
% \caption{\label{f:quad}
% The revenue curve for quadrilateral distribution $\Qr_{\qo, \qt, r}$. }
% \end{figure}
% For simplicity, if $\bar{\val}$ is normalized such that $\bar{\val} \qo = 1$, 
% we use $\Tr_{\qo}$ to denote the corresponding triangle distribution, 
% and $\Qr_{\qo, \qt, r}$ to denote the corresponding quadrilateral distribution. 
% We also use $\tri$ to denote the set of triangle distributions, 
% and $\reg$ to denote the set of regular distributions. 
% The revenue curve for quadrilateral distribution $\Qr_{\qo, \qt, r}$. 
% is depicted in \Cref{f:quad}. 
% % For notation convenience, 
% % let $\regular$ be the set of regular distributions, 
% % $\tri$ be the set of triangle distributions,
% % and $\la$ be the set of deterministic look ahead mechanisms. 

% Given any revelation mechanism $\mecha$, 
% let $\alloci(\vali, \vali[-i])$ be the allocation for agent $i$
% given the values are $\vali$ and $\vali[-i]$. 
% A family of mechanisms that are of general interests in our setting are the family of scale invariant mechanisms.
% A mechanism is scale invariant if for each agent $i$
% and any constant $\alpha > 0$, 
% $\alloci(\alpha\vali, \alpha\vali[-i]) = \alloci(\vali, \vali[-i])$. 
% In \citet{AB-18}, the authors prove that the optimal scale invariant mechanism is the optimal prior-independent mechanism among a family of 
% simple\footnote{They show that if $\lim_{\alpha\to 0} \alloci(\alpha\vali, \alpha\vali[-i])$ always exists, 
% then the optimal scale invariant mechanism is the optimal prior-independent mechanism.} mechanisms.
% In our paper, we will also focus on the family of scale invariant mechanisms, 
% and find the optimal mechanism in this family. 
% For notation convenience, we use $\scalei$ to denote the family of scale invariant mechanisms
% We conjecture that the assumption on scale invariant is not necessary for the optimality. 

% % Let $\scalei$ be the set of scale free mechanisms and $\sfl$ be the set of scale free and look ahead mechanisms. 

% % We use $\valf_{\dist}(\quant)$ to denote the value corresponds to quantile $\quant$
% % given distribution $\dist$,
% % and use $\rev_{\dist}(\quant) = \val_{\dist}(\quant) \cdot \quant$ to denote the optimal revenue of distribution $\dist$ 
% % given quantile constraint $\quant$. 





==> proofs.tex <==


\section{Proofs for \Cref{s:adversary}}
\label{a:proofsadv}
